Automated Inference of Software Library Usage Patterns

Modern software systems are increasingly dependent on third-party libraries. It is widely recognized that using mature and well-tested third-party libraries can improve developers' productivity, reduce time-to-market, and produce more reliable software. Today's open-source repositories provide a wide range of libraries that can be freely downloaded and used. However, as software libraries are documented separately but intended to be used together, developers are unlikely to fully take advantage of these reuse opportunities. In this paper, we present a novel approach to automatically identify third-party library usage patterns, i.e., collections of libraries that are commonly used together by developers. Our approach employs hierarchical clustering technique to group together software libraries based on external client usage. To evaluate our approach, we mined a large set of over 6,000 popular libraries from Maven Central Repository and investigated their usage by over 38,000 client systems from the Github repository. Our experiments show that our technique is able to detect the majority (77%) of highly consistent and cohesive library usage patterns across a considerable number of client systems.

==> sections/Approach__1_.tex <==

\section{The proposed approach}\label{sec:approach}

In this section, we present our approach, \ourtechnique, for mining library usage
patterns. Before detailing the used algorithm, we provide a brief overview of our approach and describe our visualization technique to explore the identified of library usage patterns.

\subsection{Approach Overview}\label{sec:approachOverview}

Our approach takes as input a set of popular libraries, and a wide variety of
their client systems extracted  from existing open-source repositories. The
output is a set of library usage patterns, each pattern is a collection of
libraries , organized within different layers according to their co-usage frequency.
 %patterns of libraries as described earlier, and a set of noisy libraries which are either utilities libraries or rarely used libraries.

We define a \textit{library co-usage pattern} (LCUP) as a collection of libraries that are commonly used together. %, without being almost steadily used in client programs. 
A LCUP represents an exclusive subset of libraries, distributed on different usage cohesion layers. 
A usage cohesion layer reflects the co-usage frequency between a set of libraries. 
%Formally, given a set of libraries $L$ where $L = \{l_1, ..., l_n\}$, and $dist$ is the exclusive distribution of libraries into different layers, i.e., levels of cohesion. The layers of cohesion is a subset within the set of libraries and is defined as a recursive formula. For example, starting with $L$, the iterative formula is defined as 
%
%\begin{equation}
%\left\{\begin{array}{l}
%
% layer_1= dist(L)\\
%layer_n= dist(layer_{n-1})
%
%\end{array}\right.
%\end{equation}
%where we first define the top layer as $layer_1=dist(L)$. Then, $n$ is the number of iterations of $dist$ on $L$. The layers represent the strength of the cohesion of the usage and decreases as $n$ increases. 
%
%For example, if $L$ is composed of $\{L_1, L_2, L_3\}$. Then $layer_1$ creates a cluster of $\{L_1, L_2\}$. Then, $layer_2$ creates another cluster of $\{\{L_1, L_2\}, L_3\}$. 

Indeed, similar client systems may share some domain specific libraries, but they may at the same time share some utility libraries which are more commonly used by a large number of systems. For this reason, we seek a technique that can capture co-usage relationships between libraries at different levels. 

Our approach proceeds as follows. First, the input dataset is analyzed to identify the different client systems depending on each library. 
Then, the dependency information is encoded using usage vectors. Indeed, each  library in the dataset is characterized with a usage vector which encodes information about (1) their client systems and (2) the rest of other systems in the dataset that are not using it.
Finally, we use hierarchical clustering technique based on DBSCAN to group the libraries that are most frequently co-used together by clients. 
All libraries that have no consistent usage through the client systems are isolated and considered as noisy data.
% with respect to the degree of co-usage relationships.

\subsection{Clustering Algorithm}

Our clustering is based on the algorithm DBSCAN \cite{Ester96adensity-based}. DBSCAN is a density based algorithm, i.e., the clusters are formed by recognizing dense regions of points in the search space. 
The main idea behind it, is that each point to be clustered must have at least a minimum number of points in its neighbourhood. 
This property of DBSCAN allows the clustering algorithm to filter out all points that are not located in a dense region of points in the search space. 
In other words, the algorithm clusters only relevant points and leaves out noisy points. 


This specific property explains our choice of the clustering algorithm DBSCAN to detect usage patterns of libraries. Indeed, not all libraries of the dependency dataset are to be clustered because some are simply not co-used with specific subsets of the libraries, while others are co-used with almost all the subsets of libraries.

In our approach, each library is represented as a usage vector that has constant length $l$. The vector length is the number of all client programs which use the libraries in the dataset.
\Figref{fig:methodrep} shows that the considered dataset represents 8 client systems depending on 8 third-party libraries. For an external library, $Lib_{x}$, an entry of $1$ (or $0$) in the $i^{th}$ position of its usage vector, denotes that the client system corresponding to this position depends (or does not depend) on the considered library.
Hence, summing the entries in the library's vector represents the number of its client program in the dataset. 
For instance, in \Figref{fig:methodrep}, the usage vector of {\it Lib1} shows that the four client systems {\it C1}, {\it C2}, {\it C3} and {\it C6} depend on this library. We can also see that these systems depend on other libraries including {\it Lib2, Lib3} but  none of them depends on {\it Lib5}.

DBSCAN constructs clusters of libraries by grouping libraries that are close to each other, thus forming a dense region (\ie similar libraries) in terms of their co-usage frequency. 
For this purpose, we define the Usage Similarity, $USim$ in \equref{eq:USim}, between two libraries $Lib_{i}$ and $Lib_{j}$, 
using the Jaccard similarity coefficient with regards to the client programs,
$Cl\_sys$, of $Lib_{i}$ and $Lib_{j}$.
 
The rationale behind this is that two libraries are close to each other (short distance) if they share a large subset of common client systems.    

\begin{small}
\begin{equation}
USim(Lib_i,Lib_j) =
\frac{ |Cl\_sys(Lib_i) \cap Cl\_sys(Lib_j)|}
		{|Cl\_sys(Lib_i) \cup Cl\_sys(Lib_j)|}
\label{eq:USim}
\end{equation}
\end{small}


\noindent where $Cl\_sys(Lib)$ is the set of client programs depending on the library $Lib$.
For example, the $USim$ between the libraries {\it Lib1} and {\it Lib6} in \Figref{fig:methodrep} is $\frac{2}{4}$ since these libraries have in total $4$ client programs, and $2$ of them are common for {\it Lib1} and {\it Lib6}. 
The distance between the points in the search space corresponding to two libraries $Lib_{i}$ and $Lib_{j}$ is then computed as $Dist = 1 - USim(Lib_i,Lib_j)$.

DBSCAN requires two parameters to perform the clustering. 
The first parameter is the minimum number of points in a cluster, $minP$. 
We set this parameter at $2$, so that a usage pattern must include at least two libraries of the studied dataset. 
The second parameter is, $epsilon$, the maximum distance within which two points can be considered as neighbor, each to other. 
In other words, $epsilon$ value controls the minimal density that a clustered region can have. 
The shorter is the distance between libraries within a cluster the more dens is the cluster.

However, it is insufficient merely to apply a generic algorithm like DBSCAN `out of the box'; we need to define problem-specific clustering to provide usage patterns distributed into different levels of usage cohesion. 
 
In the next subsection, we describe our adaptation to the standard DBSCAN to support hierarchical clustering based on different values for $epsilon$ to identify different usage cohesion level in the inferred patterns.

\begin{figure}[!t]
\centering
\includegraphics[width=0.95\columnwidth]{img/methrep.pdf}
\caption{The usage vector representing the dependency between eight client programs and eight libraries.}
\label{fig:methodrep}
\end{figure}



% \begin{lstlisting}
% DBSCAN(DataSet, epsilon, MinNbPts){
%    clusters <- {}    //output of the algorithm
%    noisyPoints <- {} //output of the algorithm
%    for each unvisited point P in DataSet
%       mark P as visited
%       Neighborhood_P = getNeighbors(P, epsilon)
%       if (Neighborhood_P.size) < MinNbPts
%          noisyPoints <- noisyPoints + {P}
%       else
%          currentCluster <- new cluster
%          constructCluster(P, Neighborhood_P, currentCluster, epsilon, MinNbPts)
%          clusters <- clusters + {currentCluster}
% }
% 
% constructCluster(P, Neighborhood_P, currentCluster, epsilon, MinNbPts){
%    currentCluster <- currentCluster + {P}
%    for each point Q in Neighborhood_P
%       if Q is not visited
%          mark Q as visited
%          Neighborhood_Q <- getNeighbors(Q, epsilon)
%          if Neighborhood_Q.size >= MinNbPts
%             Neighborhood_P <- Union(Neighborhood_P,Neighborhood_Q)
%       if Q is not yet member of any cluster
%       	currentCluster <- currentCluster + {Q}
% }
% 
% getNeighbors(P, epsilon){s
%     for each point Q in DataSet
%     	if DIST(P,Q) < epsilon
%     	then Q is neighbor of P.
% }
% \end{lstlisting}

\subsection{Multi-layer Clustering}

We have introduced a variant of DBSCAN (which we call $\epsilon$-DBSCAN) specifically for the library usage patterns identification problem. 
In DBSCAN, the value of the $epsilon$ parameter influences greatly the resulting clusters. A value of $0$ for $epsilon$, means that each cluster must contain only libraries that are completely similar (\ie distance among libraries belonging to the same cluster must be 0). Our idea is to `relax' the $epsilon$ parameter that controls the  constraints on the requested density within clusters. 

On the one hand, if we set $epsilon$ at fixed small value, \eg $epsilon = 0$, this will produce patterns that are very dense. Consequently, the resulted usage patterns will include only libraries that exhibit a high co-usage score. 
On the other hand, an increase of the $epsilon$ value, \eg $epsilon = 0.3$, will
result in an additional external layer of patterns that exhibit less co-usage
score. Therefore, we iteratively apply the standard DBSCAN at different levels of $epsilon$ in order to have library usage patterns organised as multi-layers, each represents a particular co-usage score.
%And it will not be easy to distinguish between complementary domain specific libraries and utilities libraries.     

%\begin{figure}[!t]
%\centering
%\fbox{\includegraphics[width=0.9\columnwidth]{img/hdbscan.png}}
%\caption{Hierarchical DBSCAN algorithm.}
%\label{fig:hdbscan}
%\end{figure}

\begin{algorithm}[t]
\caption{$\epsilon$-DBSCAN: Hierarchical DBSCAN algorithm} 
%\small
\label{algo:dbscan}
\begin{algorithmic}[1]
\STATE $\epsilon$-DBSCAN(DataSet, maxEpsilon, MinNbPts, epsilonStep)$\{$
\STATE epsinon $<$-- 0
\WHILE{epsilon $<$ maxEpsilon}
\STATE DBSCAN(DataSet, maxEpsilon, MinNbPts, epsilonStep)
\STATE clusters $<$-- DBSCAN.clusters
\STATE noisyPoints $<$-- DBSCAN.noisyPoints
\STATE compositePoints $<$-- constructPoints(clusters)
\STATE Dataset $<$-- noisyPoints + compositePoints
\STATE epsilon $<$-- epsilon + epsilonStep
\ENDWHILE 
\STATE $\}$
\STATE constructPoints(clusters)$\{$
\FOR{each C in clusters}
\STATE compositePoints $<$-- OR(all points of C)
\ENDFOR
\STATE $\}$
\end{algorithmic}
\end{algorithm}


As a result, our $\epsilon$-DBSCAN, build the clusters incrementally by relaxing the epsilon parameter, step by step. 
Algorithm \ref{algo:dbscan} shows the pseudo-code of our incremental clustering technique, $\epsilon$-DBSCAN. 
First, $\epsilon$-DBSCAN takes as input a dataset containing all the libraries and their client systems within a specific format, then it cluster them using the standard DBSCAN algorithm with epsilon value of~$0$. This step results in clusters of libraries that are always used together, as well as multiple noisy points left out. For each produced cluster, we aggregate the usage vectors of its libraries using the logical disjunction in one usage vector. Then, a new dataset is formed which includes the aggregated usage vectors and the usage vectors of noisy libraries from the previous run. This dataset is then fed back to the DBSCAN algorithm for clustering, but with a slightly higher value of epsilon, \ie $epsilon = epsilon + epsilonStep$. 
This procedure is repeated in each step until reaching $maxEpsilon$ a maximum
value for epsilon, given as a parameter.
 %This procedure will be repeated in each step until reaching the last iteration
 % where $epsilon = maxEpsilon$.% to an epsilon value of~$\alpha$. And, the clustering process is stopped when epsilon reaches a maximum value, $\beta$, given as parameter.


% \begin{lstlisting}
%
% HDBSCAN(DataSet, maxEpsilon, MinPts, espilonStep){
%   epsilon <- 0	
%   while(epsilon < maxEpsilon)
% 	DBSCAN(DataSet, epsilon, MinPts)
% 	clusters <- DBSCAN.clusters
% 	noisyPoints <- DBSCAN.noisyPoints
% 	compositePoints <- constructPoints(clusters)
% 	DataSet <- noisyPoints + compositePoints
% 	epsilon <- epsilon + epsilonStep
% }
%
% constructPoints(clusters){
%   for each C in clusters
% 	compositePoint <- OR(all points of C)
% }
%
% \end{lstlisting}



%\begin{figure}[!th]
%\centering
%\includegraphics[width=0.85\columnwidth]{figures/ClusteringExample-resized.png}
%%\vspace{-0.25cm}
%\caption{Resulting clusters of applying the incremental algorithm to libraries
%of Figure \ref{fig:methodrep}.}
%\label{fig:clusters}
%\end{figure}


For example, \Figref{fig:clusters} shows the incremental clustering of the libraries in \Figref{fig:methodrep} using $\epsilon$-DBSCAN.  
In this example, the initial dataset contains 8 libraries, {\it Lib1, ..., Lib8}, in which the $epsilon$ parameter is incremented in each step by $epselonStep = 0.25$ with the epsilon maximum value set to $maxEpsilon = 0.55$. 
As shown in \Figref{fig:clusters-a}, the first step produces two clusters at
$epsilon = 0$. The two clusters include respectively ({\it Lib1, Lib2, Lib3})
and {\it Lib4, Lib5}. These libraries are clustered at the most dense level since, in each cluster,  these libraries were frequently co-used together.
The second step is performed with $epsilon = 0.25$ as illustrated in \Figref{fig:clusters-b}. 
For this step, there is no change in the dataset since the distances are larger than 
the current $epsilon$ value. Finally at $epsilon = 0.5$, as illustrated in
\Figref{fig:clusters-c} a new cluster involving 2 density level is generated.
This cluster includes {\it Lib7} in addition to ({\it Lib1, Lib2, Lib3}) since they share 2 out of the 4 common client systems. 

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[height=0.1\textheight]{figures/fig2a}
         \caption{ $epselone = 0$}
        \label{fig:clusters-a}
    \end{subfigure}
    ~~~~~~
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[height=0.1\textheight]{figures/fig2b}
         \caption{ $epselone = 0.25$}
        \label{fig:clusters-b}
    \end{subfigure}
    ~~~~~~~~~~~~~
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[height=0.1\textheight]{figures/fig2c}
         \caption{ $epselone = 0.5$}
        \label{fig:clusters-c}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[height=0.1\textheight]{figures/fig2d}
         \caption{ $epselone = 0.75$}
        \label{fig:clusters-d}
    \end{subfigure}
    \caption{Resulting clusters of applying the incremental algorithm using $\epsilon$-DBSCAN to the library dataset presented in Figure \ref{fig:methodrep}.}
\label{fig:clusters}
\end{figure*}


We can notice that {\it Lib6} is a rarely used library and {\it Lib8} 
is a utility library used with almost all the considered client systems, showing
no particular usage trend. Thus at the last iteration of $\epsilon$-DBSCAN 
illustrated in \Figref{fig:clusters-d}, the libraries {\it Lib6} and {\it Lib8}
are left out as  noisy points since their distance from the clustered libraries is larger than the maximum epsilon value, which is $0.55$.


\subsection{Pattern Visual Exploration}
With the exponentially growing number of software libraries in the Internet, the size of possible usage patterns tends to be very large. To simplify the exploration of the inferred patterns, we opted for an interactive and user-friendly visual exploration technique. The distribution of libraries 
on different usage cohesion levels follows a hierarchical structure by inclusion
that can be visualized through a treemap layout \cite{ johnson1991tree}.
However, to better reveal the hierarchy, we opted for a circle packing visualization \cite{wang2006visualization} even if circle packing is not as space-efficient as a treemap. 


In our visualization, the libraries are represented as white dots and the clusters as circular region with deferent shades of blue.  \Figref{fig:visualization} shows an example of the circle packing visualization. 
Elements belonging to the same cluster (co-used elements) are placed at the inner periphery of the circular region representing the cluster. Thus the nesting between circular regions indicates the different clustering level.  Our visualization enables us to map different information to the graphical component of the visualization scene. For instance, library popularity can be mapped to the dot size, and the cluster cohesion can be mapped to the region color. 


The developer can use our visualization to explore the inferred patterns. The exploration is based only on pattern cohesion and the circle packing nesting.
Our visualization environment provides also an interactive navigation where the user can click on any usage pattern, i.e., cluster, to zoom in or zoom out. The visualization allows also to place the mouse over a library to get a tooltip with some more information. For example, when clicking on a library the user is redirected automatically to its artefact  home page on the Maven Central repository\footnote{http://mvnrepository.com} in order to download the library jar file. Our visualization allows also the developer to provide as input the set of libraries he is already using in his system and for which he is trying to find related and commonly used libraries. Thereafter, the entered libraries are highlighted in a different color, and the developer can start his exploration from the highlighted points.

\begin{figure}[!t]
\centering

	\includegraphics[width=0.95\linewidth]{img/packing.pdf}
	

\caption{circle packing visualization}
\label{fig:visualization}
\end{figure}

==> sections/Background.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Consistent API Usage Patterns}\label{sec:background}

Having introduced the concept of {\it Consistent API Usage Pattern}, and demonstrated its presence in well known APIs and its potential value for enhancing API documentation, this section provides formal definition of usage patterns in our work. 
   
As outlined earlier, we define an API usage pattern (UP) as a group (\ie cluster) of methods of the API of interest. Where an UP includes only methods which are accessible from client programs (\ie public methods of the API), and each UP represents an exclusive subset of the API's public methods. 
Let $\mathcal{P}$ be the set of all detected usage patterns of a given API, then our definition for API usage patterns is as follows:  %can API method can belong at maximum to one cluster: 
\begin{flalign}
	&UP = \{ ~m~ | ~m~ \in API~ \} ~\text{\it\small : m is public method}&     \\
	&\forall UP_i, UP_j \in \mathcal{P}, i \neq j \Rightarrow UP_i \cap UP_j = \phi &
%\end{center}
\end{flalign}

Still, we are interested only in consistent usage patterns. 
Ideally, a usage pattern UP is said consistent if the co-usage relations between the UP's methods remain consistent across all client methods of the UP. 
Where . 
Let $\mathcal{C}$ be the set of all identified client programs of the API of interest, and $cm(m)$ define the predicate which returns all methods in $\mathcal{C}$ that invoke (are client of) a method $m$ in the API, then the set of client methods of an UP ($cm(UP)$) is represented by the union of client methods for all methods in UP: 
\begin{flalign}
	&cm(UP) = \mathop{\cup}_{m_i \in UP} cm(m_i) \;: \forall m_j \in cm(m_i), m_j \in \mathcal{C}&
\end{flalign}
However, since    
 
\begin{figure}[h]
\centering 
\includegraphics[scale=0.5]{GroupLayout-UsagePattern}
\caption{The hierarchical cluster (\emph{Cl2}) which represents the consistent usage pattern of class {\tt GroupLayout} that we discussed in \Secref{sec:exampleSWING}: the {\it core} usage pattern of GroupLayout is represented by the cluster \emph{Cl0}, then the cluster \emph{Cl1} includes, \emph{partially}, the {\it peripheral} usage pattern of GroupLayout, and the cluster \emph{Cl2} includes it totally.}
\label{fig:clusters}
\end{figure}

-- methods which are commonly used together

-- consistency

-- hierarchical clustering


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/CaseStudy.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Validation}\label{sec:Validation}

In this section, we present the results of our evaluation of the proposed approach. 
Our study consists of several  experiments with the main objective of assessing
 whether our technique is able to
detect \emph{usage patterns of libraries} which are (\textit{i}) enough cohesive
to provide valuable information that can help to discover and pick up relevant
libraries, and (\textit{ii}) generalizable for new client programs. We also
compare the results of our technique \ourtechnique to the state-of-the-art
approach \davidtechnique \cite{david13}. \davidtechnique combines association rule
mining and collaborative filtering to to recommend libraries based on a set of
library usage patterns. For each experiment in this section, we present the
research questions to answer, the research method to address it followed by the obtained results.


\subsection{Data collection}\label{sec:dataset}


To evaluate the feasibility of our approach on real world scenarios, we carried out our empirical study on real-world Open Source Software (OSS) projects. As we described earlier, our study is based on widely used libraries collected from the popular library repository Maven and a large set of client systems collected form Github repository. Since Github is host of varying projects, to ensure validity of quality Github projects, we performed the following filtering on the dataset:

\begin{itemize}
\item \textit{Size}. We only included java projects that had more than 1,000 commits.

\item \textit{Forks}. We only include projects that are unique and not forks of other projects.

\item \textit{Maven dependent project}. Our projects only include projects that employ the maven build process (use \texttt{pom.xml} configuration file).
\end{itemize}



Each Github repository may contain multiple projects, each which may comprise of several systems. Each of these systems are dependent on
a set of maven libraries, that are defined in a\texttt{ pom.xml} file within the project.

\begin{table} [h]
\centering
\caption{Dataset used in the experiment}
\label{tab:minedLib}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Dataset} \\\midrule
%\# of github systems & 1.0    & 6.0  &  36.6  &4385.0\\
Snapshot Date & 15th January 2015\\
\# of github systems & 38,000 \\
\# of unique dependent libraries &  6,638 \\
\bottomrule
\end{tabular}
\end{table}

For client libraries, we selected the latest release of the library at that period of time. In the beginning we started with 40,936 dependent libraries. However, to remove noise, we filtered out libraries having less that 50 identifiers of methods, attributes and classes. This process removed libraries that we assume very small or partial copy of their original libraries and thus will not be relevant. Our dataset resulted in 6,638 different Maven libraries extracted from unique 38,000 client systems from Github.

The dataset is a snapshot of the projects procured as of 15th January 2015. Our dataset is very diversified as it includes a multitude of libraries and software systems from different application domains and different sizes. We found in our dataset, that the average number of used libraries per system is 10.56, while the median is 6. 


%\begin{table} [h!]
%\centering
%\caption{Statistics of the Maven library dataset size used in the experiment}
%\label{tab:minedLib}
%\begin{tabular}{@{}lcccc@{}}
%\toprule
%\multicolumn{1}{c}{} & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{mean} & \multicolumn{1}{c}{median}& \multicolumn{1}{c}{max}\\\midrule
%\# of github systems & 1.0    & 6.0  &  36.6  &4385.0\\
%\# of dependent libraries per system & 3.00   &  6.00&   10.56  & 292.00\\
%\# of maven identifiers per library &51.0  & 731.0 &4,729.0& 74,080.0\\
%\bottomrule
%\end{tabular}
%\end{table}


%#libs
%#Min. 1st Qu.  Median    Mean 3rd Qu.    Max.
%#3.00  &  4.00  &  6.00&   10.56   &10.00  & 292.00
%
%#vocab
%#Min. 1st Qu.  Median    Mean 3rd Qu.    Max.
%#51.0   236.5   731.0  4729.0  4005.0 74080.0

%#client per library
%#Min. 1st Qu.  Median    Mean 3rd Qu.    Max.
%#1.0    & 2.0    & 6.0  &  36.6 &   19.0  &4385.0





\subsection{Sensitivity Analysis}%\label{sec:evaluation-cohesion}
In the first experiment, we evaluated the sensitivity of the patterns' quality,
identified by \ourtechnique, with respect to different dataset size and different value of the maxEpsilon parameter. Thus, we aim at addressing the first research question.

\begin{itemize}
  \item \myparagraph{RQ1:} What is the impact of various experimental settings on the patterns quality? 

\end{itemize}


\subsubsection{Analysis method}\label{sec:setup}
To address our first research question \textbf{(RQ1)}, we need to evaluate whether the detected patterns are cohesive enough to exhibit informative usage relationships between specific libraries. 
Hence, we use the Pattern Usage Cohesion metric (PUC) to measure the cohesion of patterns. 

PUC was originally proposed and used in \cite{Pere07b} for assessing the usage cohesion of a service interface.
It evaluates the co-usage uniformity of an ensemble of entities, which in our
context, is a group of libraries, that forms a library usage pattern.
PUC states that a usage pattern has an ideal usage cohesion (PUC = 1) if all the pattern's libraries are 
actually always used together. PUC takes its value in the range [0..1]. The notion is that the larger the value of PUC is, 
the better the usage cohesion. The PUC for a given usage pattern \textit{p} is defined as follows:
\begin{equation}
PUC(p) = \dfrac{\sum_{cp} ratio\_used\_Libs(p,cp)}{\vert
C(p)\vert}
\label{eq:PUC}
\end{equation}
\noindent where \textit{cp} denotes a client programs of the pattern \textit{p};
\textit{ratio\_used\_Libs(p, cp)} is the ratio of libraries which belong to the
 pattern \textit{p} and are used by the client program~\textit{cp}; and $C(p)$
 is the set of all client programs of the libraries in \textit{p}.


We address our first research question \textbf{(RQ1)} in two steps, as follows. 
In the  first  step, we apply \ourtechnique to the  dataset described in \secref{sec:dataset} 
and we investigate the impact of different $maxEpsilon$ values on the PUC results of the detected patterns. 
In the second step, we investigate the scalability of our technique. We fix the $maxEpsilon$ value and we run \ourtechnique several times 
while varying the dataset size to observe the patterns cohesion and the time efficiency.


\subsubsection{Results of RQ1}\label{sec:setup}
\paragraph*{Sensitivity to maxEpsilon}
Our experiment shows that the $maxEpsilon$ parameter influences different characteristic of the inferred patterns (\ie the pattern usage cohesion, the number of inferred patterns, etc.). We can see in \Figref{fig:epsilonVScoh} that the average pattern cohesion ranges from 100\% to 50\%, while varying the maxEpsilon in [0 .. 0,95]. We notice that even when the $maxEpsilon$ reach high values, the inferred patterns conserve acceptable cohesion values. This is due to the incremental construction of the patterns that generates multiple layers of libraries, each reflected at a different density level. Thus, layers inferred at the early steps influence the overall cohesion of the final pattern. 
 \vspace{0.5cm}
\begin{figure}[!t]
\centering
\includegraphics[width=0.95\columnwidth]{img/fig3}

\caption{Effect of varying $maxEpsilon$ parameter on the average cohesion of the
identified patterns.}%\textcolor{red}{Aymen: x-axis and y-axis labels are
% missing. Please add them. If possible draw this plot and the figure 4 with r to be consistent with other figures.} 

\label{fig:epsilonVScoh}
\end{figure}

When $maxEpsilon$ is set to 1 the patterns cohesion drop down to 0. This is due to the fact that in the last step all the libraries are clustered into one usage pattern, as we can see in \Figref{fig:epsilonVSnbPatterns}.
We can also see in this figure that the number of inferred patterns increases to reach a peak of 1061 when $maxEpsilon$ is set to 0.80. 

Before the peak, we can observe that some of the existing patterns are enriched with new libraries to form new density layers. Conversely, new patterns are identified for libraries that were considered as noisy. This is since we are tolerating less density within clusters. We observe that this has an effect to increase the global number of inferred patterns. 

After the peak we observe that some of the existing patterns are merged without losing their internal structure. 
This, in turn has an effect to reduce the global number of inferred patterns.

%\vspace{0.6cm}
\begin{figure}[!t]
\centering
\includegraphics[width=0.95\columnwidth]{img/fig4}

\caption{Effect of varying $maxEpsilon$ parameter on the number of identified patterns.}
\label{fig:epsilonVSnbPatterns}
\end{figure}

Qualitatively speaking, we observed that for the low values of $epsilon$ and up to intermediate value (e.g., 0.5, 0.6) the inferred patterns are based on domain specific libraries (e.g., program analyzers {\tt jdepend}\footnote{ http://mvnrepository.com/artifact/jdepend/jdepend}, graphics manipulation {\tt batik}\footnote{ http://mvnrepository.com/artifact/batik/batik} etc.). Those patterns are characterized with an average number of client that does not exceed 50 clients per pattern. The more the $epsilon$ parameter is relaxed, the more the patterns are enriched. Starting with specific libraries, the patterns reach a step to where the patterns become enriched with utility or more generic libraries such as {\tt JUnit}\footnote{http://mvnrepository.com/artifact/junit/junit} and {\tt log4j}\footnote{ http://mvnrepository.com/artifact/org.apache.logging.log4j/log4j-api}. For visibility purpose, we do not represent in \Figref{fig:epsiloneVSnbClients} the last step where all the libraries are clustered into one usage pattern having a larger number of client systems.


%\vspace{0.6cm}
\begin{figure}[!t]
\centering
\includegraphics[width=0.95\columnwidth]{img/fig5}
%\vspace{-0.25cm}
\caption{Effect of varying $maxEpsilon$ parameter on the average number of clients per pattern.}
\label{fig:epsiloneVSnbClients}
\end{figure}

\paragraph*{Sensitivity to dataset size}
To carry out this experiment we set the $maxEpsilon$ value to 0.5, this is a
proactive choice to ensure that the pattern's library are co-used together at
least half the time.

We run \ourtechnique six times with different dataset size, each run we incremented the previously used dataset with 1000 new libraries 
and we observed the average cohesion of patterns as well as the needed time to infer them. All experiments were carried out on 
a computer with an Intel core i7-4770 CPU 3.40 GHz, with 32.0 GB RAM.


We can see in \Figref{fig:datasetVSpuc} that the shapes of the graph is consistent for the different dataset size. 
The patterns cohesion slightly increases from 79\% to stabilize at  82\% for the last three runs. Furthermore we noticed the increase 
of the number of inferred pattern from 62 in the first run with an average size of  3 library per pattern, to reach around 500 pattern 
at the last run with an average size of 5.5 libraries. This confirms that when considering more libraries \ourtechnique  is able to enrich the inferred patterns and to detect new ones.


\begin{figure}[!t]
\centering
\includegraphics[width=0.95\columnwidth]{img/datasetVSpuc}
%\vspace{-0.25cm}
\caption{Effect of varying the dataset size on the average pattern cohesion.}
\label{fig:datasetVSpuc}
\end{figure}

From the time efficiency perspective we can see in \Figref{fig:datasetVSTime}
that the execution time of  \ourtechnique  is as expected sensitive to the data set size. At the first 
run   \ourtechnique spend just 7 minutes to mine a set of 1000 libraries, while 159 minutes are needed to mine the large 
set of around 3,8000 client system and their 6,000 corresponding libraries. However, it is worth to say that even with 159 minutes 
of execution time, \ourtechnique can be considered time efficient, since the mining task is done offline once , then the inferred pattern 
are explored through our visualization tool.


\begin{figure}[!t]
\centering
\includegraphics[width=0.95\columnwidth]{img/datasetVSTime}
%\vspace{-0.25cm}
\caption{Effect of varying the dataset size on the time efficiency.}
\label{fig:datasetVSTime}
\end{figure}

 In summary, the obtained PUC for the identified usage patterns provides evidence
that exhibit consistent cohesion using our adopted $\epsilon$-DBSCAN technique. We show that at least 50\%, and up to 100\%, of the usage patterns are co-used
together. Moreover our technique is stable and time efficient when varying the
size of the mined library set.


\subsection{Evaluation of patterns cohesion}\label{sec:evaluation-cohesion}
This study aims at evaluating the cohesiveness of the identified library usage
patterns in comparison with the state-of-the-art
approache \davidtechnique. Thus, we aim at addressing the second research
question.

\begin{itemize}
  \item \myparagraph{RQ2:} To which extent are the detected library usage
  patterns cohesive as compared to those inferred with \davidtechnique ?
\end{itemize}

\subsubsection{Analysis method}\label{sec:setup}
To address our second research questions \textbf{(RQ2)} we opted for a
comparative evaluation since the comparison allow us to better position our approach and
characterize the obtained results.

We compared \ourtechnique to the most similar
approche. We re-implemented \davidtechnique  as described  in \cite{david13}. To
infere usage patterns \davidtechnique is based on  mining association rules obtained from
closed itemsets and generators as detected with the Zart algorithm
\cite{szathmary2006zart}.  We applied both \ourtechnique and
\davidtechnique to all the selected libraries of the case
study, as described in \secref{sec:dataset} then we compare the cohesion of the detected usage patterns through the two techniques, using the PUC metric. For \ourtechnique we fixed the $maxEpsilon$ value to 0.5 as explained earlier.


\subsubsection{Results of RQ2}\label{sec:setup}
To answer our research question \textbf{(RQ2)},we  analyze  the average usage 
cohesion  values  for all  detected   patterns  using  the  two compared
approaches. 

\tabref{tab:avgCohaymenAndDavid} clearly show that, in average,
\ourtechnique outperforms \davidtechnique for detecting cohesive usage patterns.
The PUC values obtained for \ourtechnique reflect very strong co-usage
relationships between the pattern's libraries. 

Regarding the number of inferred patterns, we can see that on one side our
multi-layer clustering allows detecting a reasonable number of patterns, with medium size of libraries distributed on the different layers. 
On the other side \davidtechnique infer  an abundant number of patterns, despite relying on closed itemsets and generators \cite{david13} to construct a 
compact set of association rules. The set of patterns obtained from closed itemsets and generators is supposed to be much smaller than the complete set of rules. 
However in practice the inferred patterns with \davidtechnique tends to be many and redundant with a small size (in average around 2 libraries per pattern). 
This poses a significant barriers to the practical adoption of these patterns. 

referring to the number of client per pattern, we notice that patterns inferred
with \ourtechnique are used in average within a  reasonable number of client systems that generally sharing some domain specific features. 
For \davidtechnique the inferred  patterns are used within an excessive number of client systems that share pairs or triplets of libraries which 
in most of the cases  are utility APIs such as {\tt JUnit},  {\tt log4j},   
{\tt slf4j-api},  {\tt commons-lang} and others.


\begin{table}[!t]
\setlength{\belowrulesep}{0.4pt}
\setlength{\aboverulesep}{0pt}
\begin{center}
\caption{Average cohesion and overview of the inferred usage patterns for 
\ourtechnique and \davidtechnique.
\label{tab:avgCohaymenAndDavid}}
\begin{tabular*}{1\linewidth}{ @{\extracolsep{\fill}} l|c|c}		
{\bf Number of patterns}		&	{\bf \ourtechnique}		&	{\bf \davidtechnique}	\\
\toprule
Avg PUC 						& 	0.82 		&	0.72			 \\
\midrule
Nb Paterns 						&	531		&	3952			 \\
\midrule
Avg pattern size 				&	5.5		&	2.0			  \\
\midrule
Nb Client per Pattern			&	30		&	2269			\\
\bottomrule
\end{tabular*}
\end{center}
\end{table}



\subsection{Evaluation of patterns generalization}\label{sec:evaluation-cohesion}

In study, we aim at evaluating whether we are able to generalize the identified
library usage patterns in comparison with \davidtechnique.
We aim at addressing the following research question.


\begin{itemize}
\item \myparagraph{RQ3:} To which extent the detected usage pattern could be generalized to other ``new'' client programs, that are not considered in the mining process?
\end{itemize}

\subsubsection{Analysis method}\label{sec:setup}
The setup settings described in this section were applied for the two compared.
approaches

The detection of usage patterns depends on the used set of libraries and client systems.
Hence, to address our third research question \textbf{RQ3}, we need to evaluate whether the detected patterns will have similar usage cohesion in the context of new client systems (validation client programs).  
Our hypothesis is that: 

\begin{quote}
{\it Detected patterns are said ``generalizable'' if they remain characterized
by a high usage cohesion degree in the contexts of various client systems.} 
\end{quote}

This is regardless of whether or not those client programs were used in the
detection of the patterns.
To evaluate the generalizability of the detected patterns, we perform a ten-fold cross-validations on all the client systems of the dataset. 
We randomly distribute the dataset into ten equal-sized parts. We perform ten runs of the two technique, each run uses nine parts as training client systems 
for detecting the patterns, and leaves away the remaining part as validation dataset of client systems.
 
The results are sorted in ten runs, where each run has its associated patterns, and its corresponding training and validation client programs. 
Then, we address our third question \textbf{(RQ3)} in two steps as follows. 

In the first step, We evaluate the cohesion of the detected patterns (as
measured by PUC) in the contexts of validation datasets. However, in a given run, it is possible that some detected patterns involve only 
libraries that are not used at all in the validation client programs.
Therefore, to evaluate the generalizability of the detected patterns in a run, we consider only patterns which contain at least 
one library that is actually used by the run's validation client systems. 

We call such patterns as the `eligible patterns' for the validation client systems. 
For an eligible pattern, the pattern will have a low PUC if only a small subset of its libraries are used by 
the validation client systems, while the other libraries have not been used.  As
a consequence, it will be considered as ``not generalizable''. At the end of this step, 
we compare between the PUC results obtained in the training client systems
context and validation client systems context for both \ourtechnique and \davidtechnique.


In the second step, to push further the comparison and as \davidtechnique is
specially designed for library recommendation. We tried to see if our approach
was also useful in a recommendation context. Thus we define for the libraries of
the patterns inferred by \ourtechnique an ad hoc ranking score. based on the
pattern cohesion and the library usage similarity.


for each run of the cross-validation we  tried to recommend useful libraries for
the validation client systems. For each project in the validation dataset, we
drop half of its libraries and use these as the ground truth. The remaining half are used as inputs to the recommendation process. 
This methodology was used in \cite{david13} and mimics the scenario where a developer knows some of the needed libraries but needs help to find other
relevant librairies. For each projects that should receive library
recommendations, we first identified potentially useful patterns containing any
of its used library conserved as ground truth. Then we ranked the libraries of these patents according to their maximum usage similarity with the ground truth libraries.


We  evaluated the ranking for both  \ourtechnique and \davidtechnique using the
recall rate @k  and the Mean reciprocal rank as defined below:


Consider $N$ target projects that should receive library recommendations.
For each project $P_i$, if any of the dropped libraries is found in the top-k list of recommended libraries , we count it as a hit. 
The recall rate@k is measured by the ratio of the number of hits
over the total number $N$  of considered projects.


We also used the  Mean Reciprocal Rank (MRR),\cite{} which
is a statistic for evaluating a process that produces a list of possible recommendations, MRR could
be calculated as below where  $N$ is the total number of projects that should
receive recommendations and $rank_i$ is the rank of the first
relevant recommendation for the $i^{th}$ project:


\begin{equation}
MRR=\dfrac{1}{N}\sum_{in=1}^{N}\frac{1}{rank_{i}}
\end{equation}



\subsubsection{Results of RQ3}\label{sec:setup}

\paragraph*{Patterns generalization}
We first set the $maxEpsilon$ parameter to 0.50 to ensure a sufficient 
strength of cohesion within patterns. Then, we performed the cross-validation
using both \ourtechnique and \davidtechnique.

To assess the cohesion deterioration between the training and validation client
systems, we first analyze the average value of corresponding measurements collected from all 
cross-validation runs (\tabref{tab:TrainingvsNCBValidationCoh}). Then we analyze the distribution  
of the collected values using median as depicted in (\figref{fig:Cohesion}).


\begin{table}[!t]
\setlength{\belowrulesep}{0.4pt}
\setlength{\aboverulesep}{0pt}
\begin{center}
\caption{Average Training and Validation Cohesion of identified usage 
patterns for \ourtechnique and \davidtechnique. \label{tab:TrainingvsNCBValidationCoh}}

\begin{tabular*}{1\linewidth}{ @{\extracolsep{\fill}} l||c|c||c|c}


\multicolumn{1}{c}{}				&	\multicolumn{2}{c}{{\bf \ourtechnique}} &\multicolumn{2}{c}{{\bf \davidtechnique}}\\

				\cmidrule(l{.05em}r{0.7em}){2-3}	
				\cmidrule(l{.05em}r{0.7em}){4-5}
				
				
{\bf }		&	{\bf Training}	&	{\bf Validation}	&	{\bf Training}		&	{\bf Validation}\\
{\bf PUC}	&	{\bf context}	&	{\bf context} &	{\bf context}		&   {\bf context} \\

\toprule
Avg 			&	0.77		&	0.69			&	0.72	&	0.54\\
\midrule
Max 			&	0.78		&	0.78			&	0.88 	&	0.89\\
\midrule
%Min 			&	0.73		&	0.57			& 	0.67	&	0.0\\
%\midrule
StdDev			&	0.01		&	0.05			&	0.06	&	0.27\\
\bottomrule
\end{tabular*}
\end{center}
\end{table}


\tabref{tab:TrainingvsNCBValidationCoh} summarizes the PUC of the detected patterns in the contexts of training and validation client systems. 

In the training context, we notice that the average values is high for both \ourtechnique and \davidtechnique with respectively 77\%  and 72\% of the patterns libraries 
that are co-used together. 
For \ourtechnique a slight degradation of the PUC value is observed in the
context of validation client systems. We also notice that the standard deviation values 
are very low (0.01 and 0.05). This results reflect that, overall, the  detected patterns had good PUC in the context 
of both validation and training  client systems. Whereas for \davidtechnique the average usage cohesion values are significantly 
lower in the validation context as compared to the training context.


\begin{figure}[!t]
\centering
\includegraphics[width=0.6\columnwidth]{img/Boxplotv1.pdf}
\caption{Cohesion values of identified library usage patterns in the contexts of
training and validation clients}
\label{fig:Cohesion}
\end{figure}

Moreover, the distribution of PUC values for all detected usage patterns in \figref{fig:Cohesion} confirms the above-mentioned finding. Indeed, the medians and lower quartiles in the context of validation clients remain larger than 66\%.  \figref{fig:Cohesion} also  confirms   that the  degradation  of  cohesion  values for each inferred pattern  is  much  more  visible  in the case of \davidtechnique.  

In summary we can say that almost all detected usage patterns with \ourtechnique retain their  informative criteria (precisely 75\% of detected usage patterns, according to the boxplot lower quartile), which is characterized with a high usage cohesion in both the training and validation context.

\paragraph*{Library recommendation}
\tabref{tab:recall} shows the recall rate@k for both \ourtechnique and
\davidtechnique while varying the value of k. we can see that as expected a larger k results in a higher recall rate for the two techniques. 
But more interestingly we can notice that when comparing recall rate for both \ourtechnique and \davidtechnique, the order relation is not maintained.  Indeed for the first two level \ourtechnique performs better, 
then the order is reversed in favor of \davidtechnique. This means that for most cases, good recommendations appear early in the recommendation list when using \ourtechnique. 
This hypothesis is strengthened by theresults of  MRR metric.

However good recommendation occur for more targeted client systems when using  \davidtechnique. This is mainly due to the fact that patterns inferred with \davidtechnique are mainly composed of utility libraries, unlike the pattern inferred  with \ourtechnique which are mainly composed of domain specific libraries especially  when $maxEpsilon$ values is set to low and intermediate value (e.g., 0.5).  However one can think that recommending utility libraries is less useful.
It is also worth to say that the for each fold we try to recommend useful Libraries for around 3.800 validation client system, which is huge and explains somehow the low values presented in \tabref{tab:recall} for both \ourtechnique and \davidtechnique.


\begin{table}[!t]
\setlength{\belowrulesep}{0.4pt}
\setlength{\aboverulesep}{0pt}
\begin{center}
\caption{recommendation capability for both \ourtechnique and \davidtechnique.
\label{tab:recall}}
\begin{tabular*}{1\linewidth}{ @{\extracolsep{\fill}} l|c|c}		
		&	{\bf \ourtechnique}		&	{\bf \davidtechnique}	\\
\toprule
Recall Rate@1					& 	0.12 		&	0.01			 \\
\midrule
Recall Rate@3					&	0.14		&	0.11			 \\
\midrule
Recall Rate@5 					&	0.15		&	0.19			  \\
\midrule
Recall Rate@7					&	0.17		&	0.27			\\
\midrule
Recall Rate@10					&	0.22		&	0.34			\\
\midrule
\midrule
MRR								&	0.15		&	x			\\
\bottomrule
\end{tabular*}
\end{center}
\end{table}



==> sections/Discussion__1_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}\label{sec:discussion}


We applied our approach to over 6,000 popular third-party libraries and 38,000 client systems in order to detected possible library usage patterns. The detected patterns should be informative to help developers in automatically discovering existing library sets  and therefore relieve the developers from the burden of doing so manually. More interestingly, our variant $\epsilon$-DBSCAN shows high scalability and performance with our large dataset.

The evaluation of our approach took into account the potential generalization of the identified patterns to other client systems and showed that these usage patterns remain informative for other clients. %And are very likely to be evenly detected using a different set of client programs.
One of the key contributions of this work is the adaptation of our variant $\epsilon$-DBSCAN algorithm for mining library usage patterns. We have opted for this DBSCAN-based technique rather than a standard clustering technique since DBSCAN has the notion of noise, and it widely considered robust to outliers.

The application of our technique to detect library usage patterns requires the setting of thresholds that may impact its output. 
For instance, the $maxEpsilon$ parameter in the clustering algorithm controls the cohesion (PUC) strength of the detected patterns. 
A small value leads to highly cohesive clusters which means that the detected patterns are more informative. Hence, decreasing the value of this parameter 
would result in an improvement in cohesion of the detected patterns. However, in this case the number and the consistency (generality) of the detected patterns could decrease because the highly 
cohesive detected patterns may not be shared by a large number of clients. To
ovoid bothering potential users of our approach with tuning the value of $maxEpsilon$,  we set it to a default value of 0.5 
which ensures that the libraries within patterns are at least used more frequently together than separately.

To get more qualitative sense, we describe one of the inferred patterns
identified by our technique that can fulfil the requirements of the case
scenario discussed in \Secref{sec:sakaiproject} and that provide useful libraries
for potential extensions of the system. The developer would use {\tt scheduler}{\tt
-api} and {\tt mailsender-api} rather than the {\tt quartz} and {\tt
commons-email}. This pattern has different cohesion layers, and provides at the first layer, the libraries {\tt sakai} {\tt
-calendar-api}\footnote{mvnrepository.com/artifact/org.sakaiproject.calendar/sakai-calendar-api/} and {\tt sakai-presence-api}\footnote{mvnrepository.com/artifact/org.sakaiproject.presence/sakai-presence-api/}. In the second layer, we find three libraries that are added to the pattern, namely {\tt portal-chat}\footnote{mvnrepository.com/artifact/org.sakaiproject.portal/portal-chat/}, 
{\tt
messageforums-tool}\footnote{mvnrepository.com/artifact/org.sakaiproject.msgcntr/messageforums-tool/}
and {\tt mailsender}
{\tt -api}\footnote{mvnrepository.com/artifact/org.sakaiproject.mailsender/mailsender-api/}.
At the external usage cohesion layer the {\tt scheduler-api} is added to the pattern. Indeed, these libraries have been frequently co-used in a set of 18 client systems at least in our dataset.


It is worth noticing   that we found a trade-off between the usage cohesion of the detected patterns and their generalization. Indeed, another example of more generalizable patterns that was inferred 
when $maxEpsilon$ parameter reached a relatively high value is the one formed in his core layer with some libraries of the Spring framework such 
as {\tt spring-beans }\footnote{ mvnrepository.com/artifact/org.springframework/spring-beans }, {\tt spring-context}\footnote{ mvnrepository.com/artifact/org.springframework/spring-context} 
and {\tt spring-orm}\footnote{mvnrepository.com/artifact/org.springframework/spring-orm}. Then, in the second layer, we find some libraries of the Hibernate framework such 
as the  {\tt
hibernate-
}
{\tt entitymanager}\footnote{mvnrepository.com/artifact/org.hibernate/hibernate-entitymanager}
and {\tt
hibernate-annotations}\footnote{mvnrepository.com/artifact/org.hibernate/hibernate-annotations}. Finally, in the third layer, we find some json libraries  such us the  {\tt
jackson-} {\tt databind }\footnote{
mvnrepository.com/artifact/com.fasterxml.jackson.core/jackson-databind}. The pattern continue growing until including some utility libraries of logging and testing. These libraries have been co-used in a set of hundreds of client systems.

To better assist the developers in exploring potential library usage patterns,
\ourtechnique provides a an interactive and friendly-user visualization tool. The visualization takes as input the inferred patterns and distributes them through their different layers.


==> sections/EmpiricalStudy__1_.tex <==
\section{Empirical study}\label{sec:Validation}

In this section, we present the results of our evaluation of the proposed approach, \ourtechnique. 
Our study aims at assessing whether \ourtechnique can 
detect \emph{usage patterns of libraries} that are (\textit{i})  \textit{cohesive} enough to provide valuable information to discover relevant libraries, and (\textit{ii}) \textit{generalizable} for new client systems. We also compare the results of our technique \ourtechnique to the available state-of-the-art approach, \davidtechnique \cite{david13}. \davidtechnique combines association rule
mining and collaborative filtering to recommend libraries based on their client usage. For each experiment in this section, we present the
research questions to answer, the research method to address them, followed by the obtained results.

All the material used to run our three experiments is publicly
available in a comprehensive replication package \cite{ASEdouble-blind}.

\subsection{Data collection}\label{sec:dataset}


To evaluate the feasibility of our approach on real-world scenarios, we carried
out our empirical study on a large dataset of Open Source Software (OSS)
projects. As we described earlier, our study is based on widely used libraries
collected from the popular library repository Maven and a large set of client
systems collected FROM Github repository. Since Github is the host of varying
projects, to ensure validity of quality Github projects, we performed the following filtering on the dataset:

\begin{itemize}
\item \textit{Commit size}. We only included java projects that had more than 1,000 commits.

\item \textit{Forks}. We only include projects that are unique and not forks of other projects.

\item \textit{Maven dependent project}. .   We only included projects that  employ the maven build process (use \texttt{pom.xml} configuration file).
\end{itemize}



Each Github repository may contain multiple projects, each having potentially
several  systems. Each of these systems is dependent on a set of maven libraries, that are defined in a\texttt{ pom.xml} file within the project.

\begin{table} [h]
\centering
\caption{Dataset used in the experiment}
\label{tab:minedLib}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Dataset} \\\midrule
%\# of github systems & 1.0    & 6.0  &  36.6  &4385.0\\
Snapshot Date & 15th January 2015\\
\# of github systems & 38,000 \\
\# of unique dependent libraries &  6,638 \\
\bottomrule
\end{tabular}
\end{table}

Note that for all data, we first downloaded an offline copy of the original software projects (the source code) from Github and the libraries (the jar files) from Maven before extraction. Thereafter, for each library, we selected the latest release. In the beginning we started with 40,936 dependent libraries. However, to remove noise, we filtered out libraries having less than  50 identifiers based on methods, attributes and classes. This process removed libraries that we assume very small or partial copies  of their original libraries and thus are not relevant. Our dataset resulted in 6,638 different Maven libraries extracted from unique 38,000 client systems from Github.

The dataset is a snapshot of the projects procured as of 15th January 2015. Our dataset is very diversified as it includes a multitude of libraries and software systems from different application domains and different sizes. Overall, the average number of used libraries per system is 10.56, while the median is 6. 


%\begin{table} [h!]
%\centering
%\caption{Statistics of the Maven library dataset size used in the experiment}
%\label{tab:minedLib}
%\begin{tabular}{@{}lcccc@{}}
%\toprule
%\multicolumn{1}{c}{} & \multicolumn{1}{c}{min} & \multicolumn{1}{c}{mean} & \multicolumn{1}{c}{median}& \multicolumn{1}{c}{max}\\\midrule
%\# of github systems & 1.0    & 6.0  &  36.6  &4385.0\\
%\# of dependent libraries per system & 3.00   &  6.00&   10.56  & 292.00\\
%\# of maven identifiers per library &51.0  & 731.0 &4,729.0& 74,080.0\\
%\bottomrule
%\end{tabular}
%\end{table}


%#libs
%#Min. 1st Qu.  Median    Mean 3rd Qu.    Max.
%#3.00  &  4.00  &  6.00&   10.56   &10.00  & 292.00
%
%#vocab
%#Min. 1st Qu.  Median    Mean 3rd Qu.    Max.
%#51.0   236.5   731.0  4729.0  4005.0 74080.0

%#client per library
%#Min. 1st Qu.  Median    Mean 3rd Qu.    Max.
%#1.0    & 2.0    & 6.0  &  36.6 &   19.0  &4385.0





\subsection{Sensitivity Analysis}%\label{sec:evaluation-cohesion}
As a first experiment, we evaluated the sensitivity of the patterns' quality, identified by \ourtechnique, with respect to different settings including the dataset size and $maxEpsilon$ values. We aim at addressing the following research question.

\begin{description}
\item[\textbf{RQ1.}] \textit{What is the impact of various experimental settings on the patterns'  quality?}
\end{description}


\subsubsection{Analysis method}\label{sec:setup}
To address \textbf{(RQ1)}, we need to evaluate whether the detected patterns are cohesive enough to exhibit informative co-usage relationships between specific libraries. 
Hence, we use a cohesion metric namely, Pattern Usage Cohesion metric (PUC), to capture the cohesion of the identified patterns. 

PUC is inspired from Perepletchikov et al. \cite{Pere07b} and was originally used to assess the usage cohesion of service interfaces.
It evaluates the co-usage uniformity of an ensemble of entities, which corresponds, in our context, to a set of libraries in the form of a library usage pattern.
PUC values are the range [0,1]. The larger the value of PUC is, 
the better the usage cohesion, i.e., a usage pattern has an ideal usage cohesion (PUC = 1) if all the library patterns are always used together. Let \textit{p} is a library usage pattern, then its PUC is defined as follows:
\begin{equation}
PUC(p) = \dfrac{\sum_{cp} ratio\_used\_Libs(p,cp)}{\vert
C(p)\vert} \in [0,1]
\label{eq:PUC}
\end{equation}
\noindent where \textit{cp} denotes a client system of the pattern \textit{p}, \textit{ratio\_used\_Libs(p, cp)} is the ratio of libraries that belong to the pattern \textit{p} and that are used by the client system~\textit{cp}, and $C(p)$
 is the set of all client systems of all libraries in \textit{p}.


We answer  our first research question \textbf{(RQ1)}, we perform two studies. 

\begin{itemize}
\item \textbf{Study 1.A.} We apply \ourtechnique to our collected dataset described in \secref{sec:dataset}. Then, we investigate the impact of different $maxEpsilon$ values on the PUC results of the detected patterns. 

\item \textbf{Study 1.B.} We investigate the scalability of our technique. We fix the $maxEpsilon$ value and we run \ourtechnique several times 
while varying the dataset size to observe the patterns cohesion and the time efficiency.
\end{itemize}



\subsubsection{Results for RQ1}\label{sec:setup}  


\vspace{0.2cm}

\textbf{Study 1.A: Sensitivity to \textit{maxEpsilon} parameter.}
Figures \ref{fig:epsilonVScoh}, \ref{fig:epsilonVSnbPatterns}, and \ref{fig:epsiloneVSnbClients} report the effect of different $maxEpsilon$  values. Our experiments show that the $maxEpsilon$ parameter influences different characteristic of the inferred patterns including the pattern usage cohesion, the number of inferred patterns, and the patterns size.  \Figref{fig:epsilonVScoh} shows that the average PUC ranges from 1 to 0.5, while varying the $maxEpsilon$ in the range [0,0.95]. We notice that even when the $maxEpsilon$ reaches high values, the inferred patterns maintain  acceptable cohesion values. This is due to the incremental construction of the patterns that generates multiple layers of libraries, each reflected at a different density level. Thus, layers inferred at the early steps influence the overall cohesion of the final pattern. 

%\vspace{0.5cm}
\begin{figure}[!t]
\centering
\includegraphics[width=0.95\columnwidth]{img/fig3V2}

\caption{Effect of varying $maxEpsilon$ parameter on the average cohesion of the
identified patterns.}%\textcolor{red}{Aymen: x-axis and y-axis labels are
% missing. Please add them. If possible draw this plot and the figure 4 with r to be consistent with other figures.} 

\label{fig:epsilonVScoh}
\end{figure}

When $maxEpsilon$ is set to 1 the patterns'  cohesion drop down to 0. This  is because  in the last step all the libraries are clustered into one usage pattern as depicted in \Figref{fig:epsilonVSnbPatterns}.
Moreover, we can clearly see from this figure that the number of inferred patterns increases to reach a peak of 1,061 when $maxEpsilon$ is set to 0.80. In more details, we observe that:

\begin{itemize}
\item Before the peak, some of the existing patterns are enriched with new
libraries to add new external layers to the original usage pattern. Moreover, we
 also noticed that  some new patterns are identified with libraries that were
considered as noisy. This is since we are tolerating less density within clusters when $maxEpsilon$ increases. %Aymen: I didnt understand this sentence well, how we are tolerating less density?.
 We observe that this has an effect to increase the global number of inferred patterns. 

\item After the peak, some of the existing patterns are merged without losing their internal structure. 
This result, in turn has an effect to reduce the overall number of inferred patterns.
\end{itemize}
 


%\vspace{0.6cm}
\begin{figure}[!t]
\centering
\includegraphics[width=0.95\columnwidth]{img/fig4V2}

\caption{Effect of varying \textit{maxEpsilon} parameter on the number of identified patterns.}
\vspace{0.5cm}
\label{fig:epsilonVSnbPatterns}
\end{figure}

To get more qualitative sense of the obtained results, we noticed that for the
low values of $maxEpsilon$ and up to intermediate values (i.e., 0.5, 0.6),
 %Aymen: please be a bit more precise what is low and what is inetermediate? 
 the inferred patterns tend to mainly cover domain specific libraries (e.g., program analyzers {\tt jdepend}\footnote{ http://mvnrepository.com/artifact/jdepend/jdepend}, graphics manipulation {\tt batik}\footnote{ http://mvnrepository.com/artifact/batik/batik}, etc.). Those patterns are characterized with an average number of client systems that do not exceed 50 clients per pattern. The more the $maxEpsilon$ parameter is relaxed, the more the patterns are enriched with other  libraries. Starting with specific libraries, the patterns reach a step in which they become enriched  with utility or more generic libraries such as {\tt JUnit}\footnote{http://mvnrepository.com/artifact/junit/junit} and {\tt log4j}\footnote{ http://mvnrepository.com/artifact/org.apache.logging.log4j/log4j-api}. For sake of simplicity, we do not present in \Figref{fig:epsiloneVSnbClients} the last step where all the libraries are clustered into one single usage pattern with a larger number of client systems. Based on these results, \ourtechnique uses a $maxEpsilon$ threshold of 0.5 as a defaults parameter.


\vspace{0.9cm}
\begin{figure}[!t]
\centering
\includegraphics[width=0.95\columnwidth]{img/fig5V2}
%\vspace{-0.25cm}
\caption{Effect of varying $maxEpsilon$ parameter on the average number of clients per pattern.}
\label{fig:epsiloneVSnbClients}
\end{figure}

\vspace{0.25cm}
\textbf{Study 1.B: Sensitivity to the dataset size.}
To carry out this experiment, we set the $maxEpsilon$ value to 0.5. This is a
proactive choice to ensure that libraries appearing in the same pattern are used more frequently together than separately. %Aymen: what is half the time?
Thereafter, we run \ourtechnique with different dataset sizes. In each run, we augmented  the previously used dataset with 1000 libraries, 
and we observed the average cohesion of patterns as well as the execution time taken to infer them. All experiments were carried out on 
a computer with an Intel core i7-4770 CPU 3.40 GHz, with 32 GB RAM.


\Figref{fig:datasetVSpuc} depicts the obtained results for this experiment. We noticed from the figure, that the shaps of the graph is consistent for the different dataset size. 
The PUC score slightly increases from 0.79 to stabilize at  0.82 for the last three runs. 
%79\% to stabilize at  82\% for the last three runs. 
In more details, we found that there is an increase in terms of the number of
inferred patterns from 62 in the first run with an average size of 3 libraries
per pattern, to reach the bar of 500 patterns at the last run with an average
size of 5.5 libraries per pattern. These  results confirm that when considering more libraries, \ourtechnique  is able to enrich the inferred patterns with new libraries while detecting new patterns.


\begin{figure}[]
\centering
\includegraphics[width=1\columnwidth]{figures/figure7}
%\vspace{-0.25cm}
\caption{Effect of varying the dataset size on the average pattern cohesion $maxEpsilon = 0.5$.}
\label{fig:datasetVSpuc}
\end{figure}

In terms of time efficiency, \Figref{fig:datasetVSTime} depicts the influence of
the dataset size on the execution time. As it can be seen on the figure, the
execution time of  \ourtechnique  is sensitive to the dataset size, as  expected. At the first run, \ourtechnique took less than 7 minutes to mine a set of 1,000 libraries, while reaching 159 minutes of execution time to mine the large set of 6,000 libraries with their 38,000 client systems. However, it is worth saying  that even with 159 minutes 
of execution time, \ourtechnique can be considered time efficient, since the inference process is done off-line once, then the identified patterns can be easily explored using our interactive visualization tool.


\begin{figure}[]
\centering
\includegraphics[width=1\columnwidth]{figures/figure8}
%\vspace{-0.25cm}
\caption{Effect of varying the dataset size on the time efficiency with $maxEpsilon = 0.5$.}
\label{fig:datasetVSTime}
\end{figure}

 In summary, the obtained PUC results of the identified usage patterns provide evidence
that \ourtechnique exhibits consistent cohesion using our adopted $\epsilon$-DBSCAN technique. Using a default $maxEpsilon = 0.5$, we found that at least 50\%, and up to 100\%, of the usage patterns are co-used together with high PUC. Moreover, our technique is stable and time efficient when varying the size of the mined library set.
%\textcolor{red}{More importantly, the reader expect to see here in the summary what is the best epsilon parameter that he can use by default?}


\subsection{Evaluation of patterns cohesion}\label{sec:evaluation-cohesion}
As a second experiment, we conduct a comparative study to evaluate the cohesiveness of the identified library usage patterns against the state-of-the-art approach \davidtechnique \cite{david13}. To the best of our knowledge, \davidtechnique \cite{david13} is the only existing approach that has addressed this problem. We aim at addressing the following research
question.

\begin{description}
\item[\textbf{RQ2.}] \textit{To which extent are the identified library usage patterns cohesive as compared to those inferred with \davidtechnique ?}
\end{description}

\subsubsection{Analysis method}\label{sec:setup}
To address our second research questions \textbf{(RQ2)} we conducted a
comparative evaluation of our approach with \davidtechnique in order to better position our approach and
characterize the obtained results.

To infer usage patterns, \davidtechnique is based on  mining association rules obtained from closed itemsets and generators using the Zart algorithm \cite{szathmary2006zart}.  
We applied both \ourtechnique and \davidtechnique to all the selected libraries
of our dataset (cf. \secref{sec:dataset}). Then, we compare the identified usage
patterns of both approaches in terms of PUC. More specifically, we  compare  the
average PUC  values  for all  detected   patterns  of each approach. For
\ourtechnique, we fixed the $maxEpsilon$ value to 0.5 as explained earlier. For \davidtechnique we fixed the $Minconf$ to 0.8 , the $Minsup$ to 0.002 and the $Number$ $of Nearest Neighbors$ to 25 \cite{david13}.


\subsubsection{Results for RQ2}\label{sec:setup}


\tabref{tab:avgCohaymenAndDavid} reports the obtained results for \textbf{RQ2}. On average,
\ourtechnique achieves an average PUC score of 0.82 which outperforms \davidtechnique that was only able to achieve  0.72 of PUC. 
The achieved PUC values  by \ourtechnique reflect high co-usage
relationships between the pattern's libraries making them more cohesive. 

In terms of number of inferred patterns, we observe that our
multi-layer clustering technique allows detecting a reasonable number of
patterns of 531, with a medium size of libraries distributed on the different
layers (i.e., 5.5). On the other hand, \davidtechnique inferred   an abundant number
of patterns up to 3,952, even though it relies on closed itemsets and generators  to construct a compact set of association rules \cite{david13}. Indeed, the set of patterns obtained from the closed itemsets and generators is supposed to be much smaller than the complete set of rules.
However, in practice the inferred patterns with \davidtechnique tend to be many but with smaller size (on average, it generates 2 libraries per pattern). We believe that this large number of small size library patterns will in turn limit the practical adoption and usefulness of the LibRec approach. 

Furthermore, we studied the number of clients per pattern. We noticed from the results of Table \ref{tab:avgCohaymenAndDavid}, that the patterns inferred by \ourtechnique are used on average with 30 client systems. Indeed, by manually investigating these client systems, we found that they generally share common domain specific features. 
For \davidtechnique, the inferred  patterns are used within an excessive number of client systems that share pairs or triplets of libraries which 
are, in most of the cases, utility libraries such as {\tt JUnit},  {\tt log4j},   
{\tt slf4j-api},  {\tt commons-lang} and several others. These libraries are likely to be used by several unrelated client systems.



\begin{table}[h!]
%\fontsize{6.7}{7}\selectfont
\tabcolsep=0.4cm
\centering
\caption{Average cohesion and overview of the inferred usage patterns for 
\ourtechnique and \davidtechnique.
\label{tab:avgCohaymenAndDavid}}
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Number of patterns} & \textbf{\ourtechnique} & \textbf{LibRec} \\ \midrule
Avg PUC                     & 0.82                   & 0.72            \\
Nb Patterns                  & 531                    & 3,952            \\
Avg pattern size            & 5.5                    & 2.0             \\
Nb Clients per Pattern       & 30                     & 2,269            \\ \bottomrule
\end{tabular}
\end{table}


%\begin{table}[!t]
%\setlength{\belowrulesep}{0.4pt}
%\setlength{\aboverulesep}{0pt}
%\begin{center}
%\caption{Average cohesion and overview of the inferred usage patterns for 
%\ourtechnique and \davidtechnique.
%\label{tab:avgCohaymenAndDavid}}
%\begin{tabular*}{1\linewidth}{ @{\extracolsep{\fill}} l|c|c}		
%{\bf Number of patterns}		&	{\bf \ourtechnique}		&	{\bf \davidtechnique}	\\
%\toprule
%Avg PUC 						& 	0.82 		&	0.72			 \\
%\midrule
%Nb Paterns 						&	531		&	3952			 \\
%\midrule
%Avg pattern size 				&	5.5		&	2.0			  \\
%\midrule
%Nb Client per Pattern			&	30		&	2269			\\
%\bottomrule
%\end{tabular*}
%\end{center}
%\end{table}



\subsection{Evaluation of patterns generalization}\label{sec:evaluation-cohesion}

In this study, we aim at evaluating whether the identified library usage
patterns with \ourtechnique  can be generalizable in comparison with those of 
\davidtechnique. We aim at addressing the following research question.

\begin{description}
\item[\textbf{RQ3.}] \textit{To which extent are the detected usage patterns generalizable to other  ``new'' client systems, that are not considered in the training dataset?}
\end{description}


\subsubsection{Analysis method}\label{sec:setup}

%The settings described in this section were applied for the two compared
%approaches. 

%The detection of usage patterns depends on the used set of libraries and client systems.
%Hence,

To answer \textbf{RQ3}, we investigate whether the detected patterns will have
similar PUC values in the context of new client systems. % (validation client programs).
 Our hypothesis is that: 

\begin{quote}
{\it Detected patterns are said ``generalizable'' if they remain characterized
by a high usage cohesion degree in the contexts of various client systems.} 
\end{quote}





To evaluate the generalizability of the detected patterns, we perform a ten-fold cross-validation on all the client systems in the dataset. 
We randomly distribute the dataset into ten equal-sized parts. Then, we perform ten independent runs of both approaches, \ourtechnique and \davidtechnique. Each run uses nine parts as training client systems 
to detect possible patterns, and leaves away the remaining part as a validation dataset.
 
The results are sorted in ten runs, where each run has its associated patterns, and its corresponding training and validation client systems. 
Then, we address \textbf{(RQ3)} through two experimental studies as follows. 

\begin{itemize}
\item \textbf{Study 3.A.} We evaluate the cohesion of the detected patterns (as measured by PUC) in the context of validation datasets. In a given run, it is possible that some detected patterns contain only 
libraries that are never used in the validation client systems.
Consequently, to evaluate the generalizability of the detected patterns in each run, we consider only the patterns that contain at least 
one library that is actually used by the run's validation client systems. 

We call such patterns the `\textit{eligible patterns}' for the validation client systems. 
An eligible pattern will have a low PUC if only a small subset of its libraries
is  used by the validation client systems, while the other libraries have not
been used.  As a consequence, it will be considered as ``non-generalizable''.
This study aims at comparing  the PUC results obtained for the training client
systems context and validation client systems context for both \ourtechnique and \davidtechnique.


\item \textbf{Study 3.B.} 
In this study, we push further the comparison, as \davidtechnique is
specifically designed for library recommendation. We attempt to evaluate whether our approach is also useful in a recommendation context. To this end, we define for the library patterns inferred by \ourtechnique an ad-hoc ranking score based on the pattern cohesion and the library usage similarity. %\textcolor{red}{Aymen: you have to clearly describe the ranking technique. What is `ad-hoc ranking'?}


For each fold, we identify a recommendation set of useful libraries for
the validation client systems. For each system, we drop half of its libraries and use them as the ground truth. The remaining half is used as input to the recommendation process.  This methodology was also used in \cite{david13} and mimics the scenario where a developer knows some of the useful libraries but needs assistance to find other
relevant libraries. 

For each system that should receive library
recommendation, we first identified potentially useful patterns containing at least on library from the ground truth set.
Thereafter, we rank the libraries of these patterns according to their recommendation score as defined below:
 
 \begin{equation}
RecScore(L)=\max_{i} \lbrace   USim(L,Lib_i)    /  Lib_i  \in GT  \rbrace
\end{equation}
 
 where $USim$ is the Usage Similarity in \equref{eq:USim}, and $GT$ is the set
 of libraries conserved as ground truth of the client system that should receive library recommendations.


We  evaluate the ranking for both \ourtechnique and \davidtechnique using two
metrics commonly used in recommendation systems for software
engineering \cite{Avazpour2014,tantithamthavorn2013mining,tantithamthavorn2013using}:
(\textit{i}) the recall rate@$k$, and (\textit{ii}) the Mean reciprocal rank (MRR) as follows. To measure the recall@$k$, we consider $N$ target systems $S$that should receive library recommendations.
For each system $S_i \in S$, if any of the dropped libraries is found in the top-$k$ list of recommended libraries, we count it as a hit. 
The recall rate@$k$ is measured by the ratio of the number of hits
over the total number $N$  of considered systems. Inspired by the previous studies \cite{Avazpour2014,tantithamthavorn2013mining,tantithamthavorn2013using}, we choose the $k$ value to be 1, 3, 5, 7, and 10. Formally, the recall rate@$k$ is defined as follows:

\begin{small}
\begin{equation}
Recall~rate@k(S)=\dfrac{\sum\limits_{\forall S_i \in S}isCorrect(S_i,\textrm{Top-}k)}{N}
\end{equation}
\end{small}

\noindent where the function $isCorrect(S_i,\textrm{Top-}k)$ returns a value of 1 if at least one of the top-$k$ recommended libraries is in the ground truth set, or 0  otherwise.

The MRR  is a statistic measure that is commonly used to evaluate
recommendation systems.  Let $N$ be the number of systems that should receive recommendations, and $rank_i$ is the rank of the first relevant recommendation for the $i^{th}$ system, then the MRR score is calculated as follows:
\begin{equation}
MRR=\dfrac{1}{N}\sum_{i=1}^{N}\frac{1}{rank_{i}}
\end{equation}
\end{itemize}






\subsubsection{Results for RQ3}\label{sec:setup}

\vspace{0.25cm}
\textbf{Study 3.A: Patterns generalizability.}
%We first set the $maxEpsilon$ parameter to 0.50 to ensure a sufficient  strength of cohesion within patterns. Then, we performed the cross-validation using both \ourtechnique and \davidtechnique.
To assess the PUC score variation between the training and validation client systems, we first analyze the average value of their corresponding scores collected from all cross-validation runs. Then, we analyze the distribution of the collected values using the median. The results of this study are summarized in \tabref{tab:TrainingvsNCBValidationCoh} and \figref{fig:Cohesion}.


\begin{table}[!t]
\setlength{\belowrulesep}{0.4pt}
\setlength{\aboverulesep}{0pt}
\begin{center}
\caption{Average Training and Validation Cohesion of identified usage 
patterns for \ourtechnique and \davidtechnique. \label{tab:TrainingvsNCBValidationCoh}}

\begin{tabular*}{1\linewidth}{ @{\extracolsep{\fill}} l||c|c||c|c}


\multicolumn{1}{c}{}				&	\multicolumn{2}{c}{{\bf \ourtechnique}} &\multicolumn{2}{c}{{\bf \davidtechnique}}\\

				\cmidrule(l{.05em}r{0.7em}){2-3}	
				\cmidrule(l{.05em}r{0.7em}){4-5}
				
				
{\bf }		&	{\bf Training}	&	{\bf Validation}	&	{\bf Training}		&	{\bf Validation}\\
{\bf PUC}	&	{\bf context}	&	{\bf context} &	{\bf context}		&   {\bf context} \\

\toprule
Avg 			&	0.77		&	0.69			&	0.72	&	0.54\\
\midrule
Max 			&	0.78		&	0.78			&	0.88 	&	0.89\\
\midrule
%Min 			&	0.73		&	0.57			& 	0.67	&	0.0\\
%\midrule
StdDev			&	0.01		&	0.05			&	0.06	&	0.27\\
\bottomrule
\end{tabular*}
\end{center}
\end{table}


\tabref{tab:TrainingvsNCBValidationCoh} summarizes the PUC results of the detected patterns in the contexts of training and validation client systems. 
In the training context, we notice that the average values is high for both \ourtechnique and \davidtechnique with respectively 77\%  and 72\% of the patterns libraries 
that are co-used together. 
For \ourtechnique, a slight degradation of the PUC value is observed in the
context of validation client systems. We also notice that the standard deviation values 
are very low (0.01 and 0.05). TThese results reflect that, overall, the 
detected patterns had good PUC in the context of both validation and training client systems. However, for \davidtechnique the
achieved average PUC values are significantly lower in the validation context comparing to the training context.


\begin{figure}[!t]
\centering
\includegraphics[width=0.9\columnwidth]{img/Boxplotv1.pdf}
\caption{PUC results of the identified library usage patterns in the contexts of training (T) and validation (V) clients achieved by each of \ourtechnique and \davidtechnique.}
\label{fig:Cohesion}
\end{figure}



In more details, the distribution of PUC values for all detected usage patterns in \figref{fig:Cohesion} confirms the above-mentioned finding. Indeed, the medians and lower quartiles in the context of validation clients remain larger than 66\%.  \figref{fig:Cohesion} also  provides evidence  that the  degradation  of  cohesion  values for each inferred pattern  is  much  more  visible  in the case of \davidtechnique.  

In summary, we can say that almost all detected usage patterns achieved by \ourtechnique retain their  informative criteria. Precisely, 75\% of detected usage patterns, according to the boxplot's lower quartile, are characterized with a high usage cohesion in both training and validation contexts.

\vspace{0.25cm}
\textbf{Study 3.B: Library recommendation.}
\tabref{tab:recall} reports the recall rate@$k$ for both \ourtechnique and
\davidtechnique while varying the value of $k \in \{1,3,5,7,10\}$. We notice that, as expected, larger $k$ values achieve higher recall rates for both approaches. More specifically, we can see that when comparing the recall rate,  \ourtechnique performs clearly better in terms of recall@1 and recall@3. However, the starting from $k=5$, \davidtechnique tends to achieve  better results. This indicates that \ourtechnique is more efficient in recommending correct libraries in the top ranks within the recommendation list when using \ourtechnique. The MRR results support this observation with a score of 0.15 for \ourtechnique. 
%\ourtechnique can correctly recommend the first correct libraries at lower
% ranks than \davidtechnique does.

%This means that for most cases, good recommendations appear early in the recommendation list when using \ourtechnique. This hypothesis is strengthened by the results of  MRR metric.

Conversely, good recommendations are achieved for more targeted client systems when using 
\davidtechnique. This is mainly due to the fact that \davidtechnique's patterns are mainly composed of utility libraries, unlike the \ourtechnique's patterns which are mainly composed of domain specific libraries. However, one can notice that recommending utility libraries that are commonly used is less useful in practice.
It is also worth mentioning   that  for each fold, due to the large number of systems (3,800 validation client systems) that require library recommendations, the recall values achieved by both \ourtechnique and \davidtechnique are still low (below 0.34) as reported in \tabref{tab:recall}. %although both \ourtechnique and \davidtechniqueis were able to recommend correct libraries, 





\begin{table}[]
\tabcolsep=0.5cm
\centering
\caption{Recommendation recall rate and MRR results achieved by both \ourtechnique and \davidtechnique.
\label{tab:recall}}
\begin{tabular}{@{}lcc@{}}
\toprule
          & \textbf{\ourtechnique} & \textbf{LibRec} \\ \midrule
Recall@1  & 0.12                   & 0.01            \\
Recall@3  & 0.14                   & 0.11            \\
Recall@5  & 0.15                   & 0.19            \\
Recall@7  & 0.17                   & 0.27            \\
Recall@10 & 0.22                   & 0.34            \\
MRR       & 0.15                   & 0.09               \\ \bottomrule
\end{tabular}
\end{table}



%\begin{table}[!t]
%\setlength{\belowrulesep}{0.4pt}
%\setlength{\aboverulesep}{0pt}
%\begin{center}
%\caption{recommendation capability for both \ourtechnique and \davidtechnique.
%\label{tab:recall}}
%\begin{tabular*}{1\linewidth}{ @{\extracolsep{\fill}} l|c|c}		
%		&	{\bf \ourtechnique}		&	{\bf \davidtechnique}	\\
%\toprule
%Recall Rate@1					& 	0.12 		&	0.01			 \\
%\midrule
%Recall Rate@3					&	0.14		&	0.11			 \\
%\midrule
%Recall Rate@5 					&	0.15		&	0.19			  \\
%\midrule
%Recall Rate@7					&	0.17		&	0.27			\\
%\midrule
%Recall Rate@10					&	0.22		&	0.34			\\
%\midrule
%\midrule
%MRR								&	0.15		&	x			\\
%\bottomrule
%\end{tabular*}
%\end{center}
%\end{table}

==> sections/Introduction__1_.tex <==
\section{Introduction}\label{sec:introduction}
%context
Third-party software libraries have become an integral part of modern software development. Today's software systems increasingly depend on external libraries, to reduce development time, and deliver reliable and quality software. Developers can take the benefit of freely reusing functionality provided by well-tested and mature third-party libraries and frameworks through their Application Programming Interfaces (APIs) \cite{Robil09a}. Developers have to cope with the complexity of writing their code from scratch and re-inviting the wheel by automatically identifying existing library usage patterns. %However, one of the main challenges that developers face, is understanding and selecting the relevant libraries to the implementation of their systems.

%Problem and existing work
Much research effort has been dedicated to the identification of library API usage patterns \cite{Wang:2013:MSH:2487085.2487146,Uddi12,Zhon09,SaiedSaner2015,SaiedICPC2015}. The vast majority of existing works focus on the method level within a single library. Indeed, these approaches assume that the set of relevant libraries is already known to the developer, and it is only the methods in these libraries that are unknown. However, this assumption makes the task to find relevant libraries and understand their usage trend a tedious and time-consuming activity. %This task becomes more complex especially with the number of existing software libraries that is exponentially increasing in open-source software repositories.

Today's code repositories on the Internet provide an increasingly large number of reusable software libraries with a variety of functionalities. Automatically analyzing how software projects utilize these libraries, and understanding the extent and nature of software library reuse in practice is a challenging task for developers.
Indeed, software developers can spend a considerable amount of time and effort to manually identify
libraries that are useful and relevant for the implementation of their software.
Worse yet, developers may even be unaware of the existence of these libraries. %, in particular when they are not popular.
%Aymen: your approach is based on popular libraries, righ? non-popular libraries have no clients, thus cannot be clustered?
Developers tend to implement most of their features from scratch instead of reusing functionalities provided by third-party libraries as pointed out by several researchers \cite{Uddi12,Zhon09,Ekok11}.
Therefore, we believe that identifying patterns of libraries commonly
used together, can help developers to discover and choose libraries that may be
relevant for their projects' implementation.

%Our work could be seen as a pre- phase for these previous works. And our results could be fed to existing approaches to infer how API methods belonging to different complementary libraries could be used together in client programs.

In this paper, we propose a novel approach for mining
%usage patterns of third-party software libraries.
Library Co-Usage  Patterns, namely \ourtechnique.
We define a usage pattern of libraries as a collection, with different usage
cohesion levels, of libraries that are most frequently jointly  used  in
client systems.
Our approach adopts a variant of DBSCAN, a widely used density-based  clustering algorithm, to detect candidate library usage patterns based on the analysis of their frequency and consistency of usage within a variety of client systems. Different client systems may use utility libraries (e.g., \texttt{JUnit}, \texttt{log4j}, etc.) as well as domain-specific  libraries (e.g., \texttt{httpclient}, \texttt{groovy}, \texttt{spring-context}, etc.).
%Whereas similar client programs use the same domain specific libraries but they may also share utilities libraries.
Thus, the rationale  behind the distribution on different usage cohesion levels of libraries in a pattern, is to distinguish between the most specific libraries and the less specific ones. Moreover, our approach is intended to be used first to identify patterns of particular libraries that interest a developer.
These libraries could then be fed to existing approaches \cite{Uddi12,Zhon09,SaiedSaner2015,SaiedICPC2015} to recommend particular methods to be used in different contexts. Moreover, \ourtechnique provides a user-friendly visualization tool to assist developers in exploring the different library usage patterns.

We evaluate our approach on a large dataset of over 6,000 popular libraries,
%6,638
collected from Maven Central repository\footnote{http://mvnrepository.com} and
investigated their usage from a wide range of over 38,000 client systems from
Github repository\footnote{www.github.com}, from different application domains. 
%Results show that \ourtechnique is able to detect a large number of cohesive usage patterns of libraries.
%Furthermore, to evaluate the generalization of the identified usage patterns to
% potential new client systems, we performed a ten-fold cross validations. The results show that across a considerable variability of client systems, the identified usage patterns by our approach remain cohesive.
Furthermore, we evaluated the scalability of \ourtechnique as compared to LibRec \cite{david13}, a state-of-the-art library recommendation technique based on  association rule mining and collaborative filtering. We also performed a ten-fold
cross validation  to evaluate the generalizability of the identified usage
patterns to potential new client systems. Our results show that across a considerable variability of client systems, the identified usage patterns by \ourtechnique remain more cohesive than those identified by LibRec. The main contributions of the paper can be summarized as follows:


\begin{enumerate}
\item We introduce a novel approach for mining multi-level usage patterns of libraries using an adapted hierarchical clustering technique. Our  approach is supported by a user-friendly tool 
%which is publicly available\footnote{\url{www.aymen.link}}, 
to visualize and navigate through the identified library usage
patterns \cite{ASEdouble-blind-tool}.

%\textcolor{red}{To the best of our knowledge, this is the first contribution to address the problem of mining usage patters in the library level instead of method level.}

\item We mine a large dataset of over 6,000 popular libraries from Maven
repository and investigated their usage from a wide range of over 38,000 client systems from Github.

\item We evaluate the effectiveness of our approach in terms of cohesiveness and generalizability of the identified patterns. Results show that our approach was able to identify a larger number of usage patterns, on different usage cohesion levels.

\end{enumerate}

The remainder of the paper is organized as follows.
\secref{sec:motivationExamples} motivates the usefulness of \ourtechnique with two
real-world examples. We detail our approach in \secref{sec:approach}. We present our experimental study to evaluate the proposed approach in \secref{sec:Validation}, while providing discussions in  \secref{sec:discussion}. \secref{sec:relatedWork} presents the related work. Finally, we conclude and suggest future work in \secref{sec:conclusion}. 

==> sections/RelatedWork__1_.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}\label{sec:relatedWork} % (fold)
Recently, different aspects around library usage have gained considerable
attentions.
Existing contributions can be organized into different categories according to the purpose of their proposed techniques: (\textit{i}) third-party library usage, (\textit{ii}) code completion, (\textit{iii}) library API usage example, (\textit{iv}) API usage visualization, (\textit{v}) exploration of API usage obstacles, and (\textit{vi}) mining API usage patterns.

\paragraph*{\it Third-party Usage at the Library Level}
Several work were interested to the third-party usage at the library level, but
for different purpose such as. Library refactoring \cite{penta2002knowledge},
library recommendation \cite{david13} and
library miniaturization \cite{antoniol,antoniol2003moving}. The most related to our work is the one by Thung
\etal~\cite{david13}. In this work the authors proposed a hybrid approach that combines association  rule mining and  collaborative  filtering to recommends libraries based on  their usage on similar client systems. This approach is most related to our in the sense that it is also based on library usage through their client systems dependency. However, both approaches have different purpose. Thung \etal~\cite{david13} are interested in similarity between client systems to recommend libraries based on dependency  of the most similar clients, whereas in our case we are interested in the overall libraries usage to discover multi-layers library patterns.


\paragraph*{\it Code Completion} 
Enhancing current completion systems to work more effectively with large APIs
have been investigated in
\cite{Nguy12,Bruch09,hou2011evaluation,McMi11,endrikat2014api}.
This body of work makes use of database of API usage recommendation, type hierarchy, context filtering and API methods functional roles for improving the performance of API method call completion. 
Recently, Asaduzzaman \etal \cite{asad2014} proposed a context sensitive code completion technique that uses, in addition to the aforementioned information, the context of the target method call. 
%Their technique ranks candidate methods for code completion by the similarities between their contexts and the context of the target call. 


\paragraph*{\it API Usage Example}  
A similar body of work is interested in example recommendation of API usage \cite{Wang11,Ekok11,Buse12,montandon2013documenting}. 
Existing contributions can be organized in two groups: 
IDE-based recommendation systems and JavaDoc-based recommendation systems. 
These contributions tried to instruments API documentation with usage examples 
based on a static slicing, clustering and pattern abstraction.


\paragraph*{\it API Usage Visualization} 
Other contributions tried to enhance understanding API usage through explorative
and interactive methods
\cite{Moritz13:6693127,kula2014visualizing,parnin2012crowd,de2013multi}.
This body of work described multi-dimensional exploration of API usage. 
The explored dimensions are related to the hierarchical organization of projects and APIs, metrics of API usage and API domains.
A visualisation strategy would necessarily enricher the usefulness of our
approach.



\paragraph*{\it Exploration of API Usage Obstacles} 
From another perspective, the work in \cite{hou2011obstacles,wang2013detecting} explored API usage
obstacles through analyzing developers questions in  Q\&A website. 
This allows API designers to understand the problems faced while using their API, and to make corresponding improvements.




\paragraph*{\it Mining API Usage Patterns}  
Other contributions related  to ours are those interested
in mining API usage patterns \cite{Wang:2013:MSH:2487085.2487146,Uddi12,Zhon09,li2005pr}.
These contributions adopted different categories of API usage patterns, different techniques for inferring patterns and different ways to assess patterns correctness and usefulness. 
The most prominent categories are temporal (\cite{Uddi12}), unordered
(\cite{li2005pr}) and sequential (\cite{Wang:2013:MSH:2487085.2487146,Zhon09})
usage patterns. These categories were assessed through consistency, coverage and
succinctness of the mined usage patterns. Zhong \etal~\cite{Zhon09} developed the MAPO tool for mining sequential API
  usage patterns. MAPO clusters frequent API
  method call sequences extracted from code snippets, based on the number of
  called API methods and textual similarity of class and method names between
  different snippets. Our  work consider a different  level  of  granularity 
  from  these   existing works. Previous approaches infer API usage patterns at the API element level (i.e. methods call). 
  In our case we are interested in inferring usage pattern at the granularity of entire library. Past approaches assume that the developer already selected the relevant 
  library and he only need to learn how to use the methods in this library. Our work does not make  this  assumption,  and  thus  complements  the existing studies. Indeed, our approach could be used as an early phase to infer set of library consistently co-used together. Then existing approaches could be applied to learn how to use particular methods within the patterns' libraries.
  



  
%Different aspects of APIs gained a considerable attention in recent-year
%research, and  several directions have been investigated.
%
%More specifically, some  contributions
%\cite{Nguy12,Bruch09,hou2011evaluation}are related to code-completion, they tried to enhance the current completion systems to work more effectively with large APIs.
%These contributions make use of database of  API usage recommendation, type
%hierarchy, context filtering and API methods functional roles to reduces the number of API metheds proposals while using Code Completion.
%
% 
%Other studies \cite{Wang11,Ekok11,Buse12,montandon2013documenting}, were
%interested in API usage example recommendation. They can be organized in two 
%groups: IDE-based recommendation systems and JavaDoc-based recommendation systems.
%These contributions tried to instruments API documentation with usage examples 
%based on a static slicing, clustering and pattern abstraction.
%
%In \cite{hou2011obstacles,wang2013detecting}, the authors explored API usage
%obstacles through analyzing developers questions in  Q\&A website.
%This allow API designers to understand the problems faced while
%using their API, and to make corresponding improvements.
%
%Other contributions \cite{Moritz13:6693127,de2013multi} are related to API usage
%visualization. They tried to enhance understanding API usage through explorative
%and interactive methods. The authors described 
%multi-dimensional exploration of API usage. 
%The explored dimension were related to  
%the hierarchical organization of projects and APIs, metrics of API usage and API domains.
%
%
% The most
%related contributions to ours
%\cite{Wang:2013:MSH:2487085.2487146,Uddi12,Zhon09}, were interested in API usage patterns mining.
%They adopted different categories of API usage patterns, 
%different techniques for inferring patterns and different ways to assess patterns
%correctness and usefulness. The most prominent categories are temporal, unordered and sequential usage patterns. These categories were assessed through 
%consistency, coverage and  succinctness of the mined usage patterns. 
%The main limitations of theses contributions are the inability to detect less common API usage scenarios 
%and the context dependency. 
%
%Our approach tries to circumvent the limitations of the above-mentioned
%  contributions. First, we make use of multiple clients of the studied
%  API which guarantees that usage patterns are genuine and recovered from the actual
%  use of the API. Second, the hierarchical construction of our usage patterns
%  enables the identification of core usage patterns as well as
%  peripheral usage patterns independently from usage context. Finally, our
%  approach detects consistent usage patterns, since they have been used almost
%  in the same way by the majority of the client programs.

% Helping developer to learn using an API gained a considerable attention in
% recent-year research. Several directions have been investigated, in particular, code search and
% completion (\cite{Nguy12}, \cite{Wang11}, \cite{Ekok11}, \cite{McMi11},
% \cite{Bruch09}), API usage pattern mining (\cite{Achar07},
% \cite{Wang:2013:MSH:2487085.2487146}, \cite{Mich99}) and API documentation
% (\cite{Hoff03}, \cite{Hori10}, \cite{Buse12}, \cite{Deke09}, \cite{Montan13:6671315}). 
% For the sake of space, we limit our discussion to some of these contributions.
% 
%  Uddin et al.~\cite{Uddi12} detect temporal patterns of API use in terms of
%   their time of addition/removal into the source code during the client program
%   development. The fact that the detection is based on the change history of a
%   client, may introduce some imprecision in this approach due to the volatile
%   nature of the development process.
  
  
%  assume that
%  the functionality offered by an API is not always accessed uniformly
%  throughout the lifetime of a client program.
%   They tried to
%   They detect concepts as distinct groups of API functionality from the change
%   history of a client program, and then infer a temporal order between those
%   concepts to build the temporal patterns. The detected concept are , but during the development process  a
%   developer could  go through a learning phase or progressive construction
%   phase in which  he can add calls to API method then remove and/or change
%   them.
%   This may introduce miss learned information on the inferred concept.
%   On the other hand the authors use a single client program to detect usage
%   concepts which makes them non generalizable or with low consistency.

%   Zhong et al.~\cite{Zhon09} developed a tool called MAPO for mining API usage
%   patterns from the code snippets. MAPO clusters frequent API
%   method call sequences extracted from code snippets, based on the number of
%   called API methods and textual similarity of class and method names between
%   different snippets. Clustering only frequent call sequences could not be enough to detect
%   less common API usage scenarios. Moreover, textual similarity can be a barrier,
%   since it is very common that snippets with different usage contexts refer to
%   the same usage pattern.

%    which describes that in a certain usage scenario,
%   some API methods are frequently called together,  . This gap is
%   overcome in our approach since the incremental API method clustering and the
%   hierarchical patterns representation exposes both conventional API usage
%   scenarios and alternative less common scenarios.
%   Moreover textual similarity can be a barrier, since it is very common that
%   snippets without textual similarity refer the usage patterns.

%  Moritz et al.~\cite{Moritz13:6693127} present a technique for automatically
%  mining and visualizing API usage examples that occur across several functions
%  in a program. This approach represents software as a Relational Topic Model,
%  where API calls and the functions that use them are modeled as a document
%  network. The used model prevents finding common and consistent use, because no
%  links can be represented between functions belonging to different client
%  programs.



%%%%%%%%%%%%End Related Works%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/ResultsAnalysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results Analysis}\label{sec:resultsAnalysis}

%
\subsection{Patterns Cohesion (RQ1)}\label{sec:ResultsCohesion}
To answer this research question, we investigate the sensitivity of our
technique to the  maxEpsilon parameter

\begin{figure}[!th]
\centering
\includegraphics[width=0.85\columnwidth]{img/epsilonVScohesion.png}
%\vspace{-0.25cm}
\caption{Effect of varying maxEpsilon parameter on the average cohesion of identified patterns.}
\label{fig:epsilonVScoh}
\end{figure}


\begin{figure}[!th]
\centering
\includegraphics[width=0.85\columnwidth]{img/epsilonVSNBpatterns.png}
%\vspace{-0.25cm}
\caption{Effect of varying maxEpsilon parameter on the number of identified patterns.}
\label{fig:epsilonVSnbPatterns}
\end{figure}

\begin{figure}[!th]
\centering
\includegraphics[width=0.85\columnwidth]{img/epsiloneVSnbClients.png}
%\vspace{-0.25cm}
\caption{Effect of varying maxEpsilon parameter on the average number of clients per pattern.}
\label{fig:epsilonVSnbPatterns}
\end{figure}

\subsection{Patterns Generalization (RQ2)}\label{sec:ResultsGeneralization}


\begin{table}[!t]
\setlength{\belowrulesep}{0.4pt}
\setlength{\aboverulesep}{0pt}
\begin{center}
\caption{Average Training and Validation Cohesion of identified 
patterns \label{tab:TrainingvsNCBValidationCoh}}
\begin{tabular*}{1\linewidth}{ @{\extracolsep{\fill}} l|c|c}		
{\bf API}		&	{\bf Training context}		&	{\bf Validation context}	\\
\toprule
Avg 					& 	0.77 		&	0.69			 \\
\midrule
Max 					&	0.78		&	0.78			 \\
\midrule
Min 					&	0.73		&	0.57			  \\
\midrule
StdDev					&	0.003		&	0.05			\\
\bottomrule
\end{tabular*}
\end{center}
\end{table}


\begin{figure}[!t]
\centering
\includegraphics[width=0.9\columnwidth]{img/boxplot1.pdf}
\vspace{-0.25cm}
\caption{Cohesion values of identified API usage patterns in the contexts of
training and validation clients}
\label{fig:nbUPimpact}
\end{figure}



\begin{table}[!t]
\setlength{\belowrulesep}{0.4pt}
\setlength{\aboverulesep}{0pt}
\begin{center}
\caption{Number of identified pattern in the training context and number of
eligible patterns in the validation context
\label{tab:TrainingvsNCBValidationNBpatterns}}
\begin{tabular*}{1\linewidth}{ @{\extracolsep{\fill}} l|c|c}		
{\bf API}		&	{\bf Training context}		&	{\bf Validation context}	\\
\toprule
Avg 					& 	294 		&	168			 \\
\midrule
Max 					&	336		&	220			 \\
\midrule
Min 					&	262		&	121			  \\
\midrule
StdDev					&	19		&	33			\\
\bottomrule
\end{tabular*}
\end{center}
\end{table}

\begin{figure}[!t]
\centering
\includegraphics[width=0.9\columnwidth]{img/boxplot2.pdf}
\vspace{-0.25cm}
\caption{{\it Number} of inferred patterns compared to number of eligible 
patterns.}
\label{fig:nbUPimpact}
\end{figure}


\subsection{Comparative Evaluation (RQ3)}\label{sec:ResultsGeneralization}


%#################################################



==> sections/Threats.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Threats to Validity}\label{sec:threats}

\todo{\bf Hani + Houari}

%%%%%%%%%%%%End Treats to Validity%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/Validation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results Analysis}\label{sec:resultsAnalysis}

%
\subsection{Patterns Cohesion (RQ1)}\label{sec:ResultsCohesion}
To answer this research question, we investigate the sensitivity of our
technique to the  maxEpsilon parameter

\begin{figure}[!th]
\centering
\includegraphics[width=0.85\columnwidth]{img/epsilonVScohesion.png}
%\vspace{-0.25cm}
\caption{Effect of varying maxEpsilon parameter on the average cohesion of identified patterns.}
\label{fig:epsilonVScoh}
\end{figure}


\begin{figure}[!th]
\centering
\includegraphics[width=0.85\columnwidth]{img/epsilonVSNBpatterns.png}
%\vspace{-0.25cm}
\caption{Effect of varying maxEpsilon parameter on the number of identified patterns.}
\label{fig:epsilonVSnbPatterns}
\end{figure}

\begin{figure}[!th]
\centering
\includegraphics[width=0.85\columnwidth]{img/epsiloneVSnbClients.png}
%\vspace{-0.25cm}
\caption{Effect of varying maxEpsilon parameter on the average number of clients per pattern.}
\label{fig:epsilonVSnbPatterns}
\end{figure}

\subsection{Patterns Generalization (RQ2)}\label{sec:ResultsGeneralization}


\begin{table}[!t]
\setlength{\belowrulesep}{0.4pt}
\setlength{\aboverulesep}{0pt}
\begin{center}
\caption{Average Training and Validation Cohesion of identified 
patterns \label{tab:TrainingvsNCBValidationCoh}}
\begin{tabular*}{1\linewidth}{ @{\extracolsep{\fill}} l|c|c}		
{\bf API}		&	{\bf Training context}		&	{\bf Validation context}	\\
\toprule
Avg 					& 	0.77 		&	0.69			 \\
\midrule
Max 					&	0.78		&	0.78			 \\
\midrule
Min 					&	0.73		&	0.57			  \\
\midrule
StdDev					&	0.003		&	0.05			\\
\bottomrule
\end{tabular*}
\end{center}
\end{table}


\begin{figure}[!t]
\centering
\includegraphics[width=0.9\columnwidth]{img/boxplot1.pdf}
\vspace{-0.25cm}
\caption{Cohesion values of identified API usage patterns in the contexts of
training and validation clients}
\label{fig:nbUPimpact}
\end{figure}



\begin{table}[!t]
\setlength{\belowrulesep}{0.4pt}
\setlength{\aboverulesep}{0pt}
\begin{center}
\caption{Number of identified pattern in the training context and number of
eligible patterns in the validation context
\label{tab:TrainingvsNCBValidationNBpatterns}}
\begin{tabular*}{1\linewidth}{ @{\extracolsep{\fill}} l|c|c}		
{\bf API}		&	{\bf Training context}		&	{\bf Validation context}	\\
\toprule
Avg 					& 	294 		&	168			 \\
\midrule
Max 					&	336		&	220			 \\
\midrule
Min 					&	262		&	121			  \\
\midrule
StdDev					&	19		&	33			\\
\bottomrule
\end{tabular*}
\end{center}
\end{table}

\begin{figure}[!t]
\centering
\includegraphics[width=0.9\columnwidth]{img/boxplot2.pdf}
\vspace{-0.25cm}
\caption{{\it Number} of inferred patterns compared to number of eligible 
patterns.}
\label{fig:nbUPimpact}
\end{figure}


\subsection{Comparative Evaluation (RQ3)}\label{sec:ResultsGeneralization}


%#################################################



==> sections/obsoleteCaseStudy.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation}\label{sec:Validation}
%\ha{I revised the following paragraphs}

The objective of our study is to evaluate whether our technique can detect API usage patterns which are {\it consistent} independently of the API usage contexts, and which are enough cohesive to provide valuable documentation that can help in learning and using APIs.
We formulated the research questions of our study as follows:

%The main objective of our study is to evaluate whether the Incremental or
%hierarchical analysis of an API, taking into consideration a number of
%its clients program, will provide consistent and informative previews to learn
%and use the API. In our study, we address the following research questions:


\begin{itemize}
  \item \myparagraph{RQ1:} to which extent the detected API usage patterns are consistent across the API's clients?

%  \item \myparagraph{RQ2:} to which extent detected usage patterns are informative to enhance the API documentation?
	\item \myparagraph{RQ2:} to which extent the detected usage patterns are cohesive, and what is the precision of our technique in detecting high cohesive usage patterns?
\end{itemize}




\subsection{Case Study}\label{sec:caseStudy}
%To answer these research questions, we applied our technique on four widely used APIs, that we believe enough large to learn in a short time: HttpClient, Java Security, Swing and AWT (Table~\ref{tab:SelectedAPIs}).
We evaluate our technique through the usage of four widely used APIs: HttpClient, Java Security, Swing and AWT (Table~\ref{tab:SelectedAPIs}).
We used the HttpClient and Java Security APIs since they were used in the recent work by Uddin \etal \cite{Uddi12} to evaluate their technique for detecting {\it temporal} API usage pattern.
We used the Swing and AWT APIs since they are large APIs, and are widely used for developing GUIs in Java applications.
To perform our study, we selected 22 client programs for the Swing and AWT APIs, and 12 client programs for the HttpClient and Java Security APIs (see Table~\ref{tab:clients}).

%We applied our technique on four APIs that were widely used in different clients
%and that were difficult to learn in a short time. The selected APIs are enumerated
%in Table~\ref{tab:SelectedAPIs}. we selected around 20 client program for the Swing and AWT
%APIs (see Table~\ref{tab:clientSwingAwt}) and around 10 client program for the HttpClient and
%Java Security APIs (see Table~\ref{tab:clientHttpClient}).


\begin{table}[!t]
\begin{center}
\setlength{\belowrulesep}{0.4pt}
\setlength{\aboverulesep}{0pt}
\setlength\tabcolsep{0pt}
\begin{tabular*}{1\linewidth}{ %@{\extracolsep{\fill}}
	p{0.2\linewidth}|@{\quad}p{0.76\linewidth}}
{\bf API}		&	{\bf Description}	
\\
\toprule
Java Security 	& Provides features to improve security of Java applications
\\
\midrule
HttpClient 		& Implements standards for accessing resources via HTTP
\\
\midrule
Swing 			& An API providing a graphical user interface (GUI) for Java programs
\\
\midrule
AWT 			& An API for providing a platform dependent graphical user interface (GUI) for a Java program
\\
\bottomrule
\end{tabular*}
\end{center}
\vspace{-0.3cm}
\caption{Selected APIs for the Case Study}
\label{tab:SelectedAPIs}
\end{table}



%\begin{table}[!h]
%\begin{center}
%
%\begin{tabular}{|l|p{3.5cm}|c|c|}
%\hline
%API & Description & coverage of  & NB usage  \\
%	&			 &	public method & pattern \\
%\hline
%Java Security & Provides features to improve security of Java applications.  & 125 & 12 \\
%\hline
%HttpClient & Implement standards for accessing resources via HTTP & 343 & 20 \\
%\hline
%Swing & An API providing a graphical user interface (GUI) for Java programs & 1618 & 102 \\
%\hline
%AWT & An API for providing a platform dependent graphical user interface (GUI) for a Java program. & 1019 & 75 \\
%\hline
%\end{tabular}
%
%\end{center}
%\caption{Selected APIs for the Case Study}
%\label{tab:SelectedAPIs}
%\end{table}


\begin{table*}[!t]
\setlength{\belowrulesep}{0.4pt}
\setlength{\aboverulesep}{0pt}
\newcolumntype{A}{ >{\centering\arraybackslash} m{0.1\linewidth}}
\begin{center}
\setlength\tabcolsep{0pt}
\begin{tabular*}{1\linewidth}{ %@{\extracolsep{\fill}}
		A p{0.2\linewidth}|@{\quad}p{0.68\linewidth}}
%\begin{tabular}{|l|p{8cm}|}
{\bf APIs}			
	&		{\bf Client programs}			&		{\bf Description} \\
\toprule
\multirow{22}{*}{\bf\rotatebox{90}{\normalsize Swing \& AWT}} 		
	&G4P (GUI for processing) 				& A library that provides a rich collection of 2D GUI controls \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Valkyrie RCP 							& A Spring port of the current Spring Rich Client codebase. \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&GLIPS Graffiti editor 					& A cross-platform SVG graphics editor \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Mogwai Java Tools 						& Java 2D and 3D visual entity relationship design and
modeling (ERD,SQL) \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Violet	 								& An UML editor \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Mobile Atlas Creator 					& This application creates off-line raster maps \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Metawidget 							& A smart widget Building User Interfaces for domain objects \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Art-of-Illusion 						& A 3D modelling and rendering studio \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&VASSAL								 	& An engine for building and playing human-vs-human games \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Neuroph								& A lightweight Java Neural Network Framework \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&WoPeD									& A Java-based graphical workflow process editor, simulator and analyzer \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&jEdit									& A mature programmer's text editor \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Spring-RCP								& Provide a way to build highly-configurable, GUI-standards \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&GanttProject core						& An application for project management and scheduling \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Pert 									& The PERT plugin for GanttProject \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Htmlpdf 								& The html and pdf export plugin for GanttProject \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Msproject 								& MS-Project import/export plugin  for GanttProject \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&swingx 								& Contains extensions to the Swing GUI toolkit \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&JHotDraw 								& A Java GUI framework for technical and structured Graphics \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&RapidMiner 							& An integrated environment for machine learning and data mining \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Sweet Home 3D 							& An interior design application \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&LaTeXDraw 								& Is a graphical drawing editor for LaTeX \\
\bottomrule
\bottomrule
%%%%%%%%%%%%%%%%%%%%%%%%
%HttpClient \& Java Security
%%%%%%%%%%%%%%%%%%%%%%%
\multirow{12}{*}{\bf\rotatebox{90}{\normalsize HttpClient \& Java Security}}
	&Jakarta Cactus							& A simple test framework for unit testing server-side java code \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Apache JMeter 							& A project that can be used as a load testing and measure performance tool \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Heritrix 								& A web crawler \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&HtmlUnit 								& A GUI-Less browser for Java programs \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&OpenLaszlo 							& An open source platform for the development and delivery of rich Internet applications \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Mule 									& A lightweight enterprise service bus (ESB) and integration framework \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&RSSOwl									& An aggregator for RSS and Atom News feeds. \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Apache Jackrabbit 						& Is an open source content repository for the Java platform. \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&Axis2 									& A core engine for Web services. \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&RESTEasy 								& A JBoss project that provides various frameworks to build RESTful Web Services \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&WildFly 								& An application server \\
%\midrule
\cmidrule[1pt](l{0em}r{0em}){2-3}
	&WSO2 Carbon 							& An SOA middleware platform \\
\bottomrule
\end{tabular*}
\end{center}
\vspace{-0.3cm}
\caption{Client programs used in our case-study}
\label{tab:clients}
\end{table*}



%\begin{table*}[t]
%\begin{center}
%
%\begin{tabular}{|l|p{8cm}|}
%\hline
%Client programs & Description \\
%\hline
%Jakarta Cactus & is a simple test framework for unit testing server-side java code \\
%\hline
%Apache JMeter & project that can be used as a load testing and measure performance tool \\
%\hline
%Heritrix & Is a web crawler \\
%\hline
%HtmlUnit & Is an open source platform for the development and delivery of rich Internet applications \\
%\hline
%OpenLaszlo & Is an open source platform for the development and delivery of rich Internet applications \\
%\hline
%Mule & Is a lightweight enterprise service bus (ESB) and integration framework \\
%\hline
%RSSOwl & An aggregator for RSS and Atom News feeds. \\
%\hline
%Apache Jackrabbit & Is an open source content repository for the Java platform. \\
%\hline
%Axis2 & A core engine for Web services. \\
%\hline
%RESTEasy & Is a JBoss project that provides various frameworks to build RESTful Web Services \\
%\hline
%WildFly & Is an application server \\
%\hline
%WSO2 Carbon & Is an SOA middleware platform \\
%\hline
%\end{tabular}
%
%\end{center}
%\caption{Client programs used for HttpClient and java.security}
%\label{tab:clientHttpClient}
%\end{table*}



\subsection{Experimental Setup}\label{sec:setup}
To address our research questions we perform leave-one-out cross-validations for all the selected APIs of the case study, using the API's clients described in \tabref{tab:clients}.
The following describes the process of our experiments for a given API of the case study.

In the first step, let N represent the number of used clients for the considered API (\eg N = 22 for Swing), we perform N runs of our technique on the API.
Each run uses N-1 client programs as training set for detecting usage patterns, and leaves away one of the API's client programs as validation set.
The results of this step are N runs, where each run has its associated usage patterns, and its corresponding training and validation sets.
In the second step, for each run we evaluate the consistency of the detected usage patterns between the training set and the validation set, and we evaluate the cohesiveness of the detected usage patterns in the contexts of training and validation sets.
		
		
A pattern is said consistent if the co-usage relationships between the pattern's methods in the context of the training set remain the same (or very similar) in the context of the validation set.
However, in a given run, it is possible that some methods involved in the detected usage patterns are not used at all in the validation set.
Therefore, to evaluate the consistency of detected patterns in a run, we consider only patterns which contain at least one method that is actually used by the run's validation set.
We call such patterns as the eligible patterns for the validation set.
However, if only a small subset of the eligible pattern's methods are used by the validation set, while the other methods of this pattern are not used, then this eligible pattern will be evaluated as inconsistent.

As for the cohesion property, in each run we evaluate the usage cohesion of
detected patterns in the contexts of both training and validation sets.
Our hypothesis is: the consistent API usage patterns can contribute to the API documentation if they remain   characterized by a high usage cohesion degree in the contexts of various API clients, regardless of the natures and features of those clients, and even though those clients were not used for detecting the patterns.
Hence, in each leave-one-out run, we evaluate the precision of our technique as the ratio of highly cohesive patterns in the context of the run's validation set.



\subsection{Metrics}\label{sec:Metrics}
To measure the co-usage relationships between the methods of a generated usage pattern, we use the Service Usage Cohesion Metric (SIUC), taken from Perepletchikov \etal \cite{Pere07b,Pere10a}.
SIUC was recently used in other work \cite{Abde13x,Dani11a} to measure the usage cohesion of interfaces in Java OO applications, where, like our definition of a usage pattern, an interface is defined as a group of method declarations.
However, in this cited body of work, the clients of an interface are computed at class granularity (\ie clients are classes), while in our work, the clients of a pattern are methods (\ie clients are computed at method granularity).
In the following, we refer to the SIUC metric as Pattern Usage Cohesion (PUC).
The metric is defined as follows:

\begin{equation}
PUC(p) = \dfrac{\sum_{c} \dfrac{num\_used\_mtds(p,c)}{size(p)}}{\vert
cm(p)\vert}  \vee c \in  cm(p)
\label{eq:PUC}
\end{equation}
Where \textit{c} denotes a client method of the pattern \textit{p};
\textit{num\_used\_mtds(p, c)} is the number of API�s methods which belong to the
usage pattern \textit{p} and are used by the client method~\textit{c}; and
$cm(p)$ is the set of all client methods of the usage pattern \textit{p}.
$PUC$ takes its value in the range [0..1].
The larger the value of $PUC$, the better the usage cohesion is.
$PUC$ states that a usage pattern has an ideal usage cohesion ($PUC = 1$) if all the pattern's methods are actually always used together with regard to all their client methods.

Back to our definition of consistency, the objective is to see whether the detected usage patterns for an  API, based on a set of clients (training set), will behave in a similar way with a new client program of the API (validation client), in terms of their usage cohesion.
Hence, we define the consistency of a usage pattern as:

 \begin{equation}
Consistency(p) = 1 - \vert PUC_{T}(p) - PUC_{V}(p) \vert
\label{eq:Consist}
\end{equation}
Where  $PUC_{T}$ and $PUC_{V}$ are the usage cohesion values of the pattern {\it p} in the training set context and validation set context, respectively.
This metric takes its value in the range [0..1].
A value close to 1 indicates that the co-usage relationships between the pattern's methods remain the same between training clients and the {\it ``new''} validation client, while a value close to 0 indicates a dissimilar behavior of the pattern between the two sets of clients.
%It is obvious that these metrics are calculated only for what we call eligible pattern, which is a usage pattern with at least one of its components methods is used in the new client program.
We use this metric to answer our first research question \textbf{(RQ1)}.




From another perspective, to answer our second research question \textbf{(RQ2)}, we need to evaluate whether detected usage patterns with our technique are enough cohesive to help in enhancing the API documentation.
For this purpose, we separately observed the two components of the consistency
metric:
the usage cohesion of detected patterns in the context of both training clients ($PUC_T$) and validation clients ($PUC_V$).
This is necessary because the consistency metric reflects only the behavioral similarity of detected patterns regarding the training clients and the validation client.
%In other words, if a detected usage pattern describes API methods which do not exhibits good co-usage relationships (\ie it is characterized with poor usage cohesion) for both the training clients and the validation clients, this means that this usage pattern is characterized with a good consistency.
%However, such a usage pattern is not informative since it does not provide valuable information regarding co-usage relationships between the API methods.
%Hence, at this stage of the validation, we want to observe whether the usage cohesion of generated usage patterns is good enough to reveal informative patterns that could be useful for the API documentation.

Observing a variety of generated usage patterns for all studied APIs, we found that a usage pattern is informative enough for documenting the co-usage relationships between the API methods if the pattern's usage cohesion value (as measured by \equref{eq:PUC}) is larger than 0.75.
Indeed, roughly speaking, a $PUC(p)$ value that is equal to 0.75 is interpreted as follows: On average, at least $75\%$ of the $p$'s methods are co-used together in all usage contexts of the $p$'s methods.
Using this threshold for $PUC$'s values, we evaluated the precision of our technique for identifying informative usage patterns by the normalized ratio of generated (eligible) usage patterns which are informative in the context of both training clients (\ie $PUC_T > 0.75$) and validation clients (\ie $PUC_V > 0.75$).
Let $EP$ and $IP$ denote, respectively, the sets of eligible patterns and informative patterns, then we evaluate the precision of our technique in each run as follows:

\begin{equation}
Precision = \dfrac{\vert EP \cap IP \vert}{\vert EP \vert}
\label{eq:Precision}
\end{equation}


% \ha{I stopped here}

%In the last step of our evaluation we tried to find out to which extent the detected usage patterns was good and informative. For this we dissected the consistency metric and we separately observed its two components PUCt and PUCv.
%
%In fact, this was necessary because the consistency metric reflected only the behavioral similarity of the pattern regarding the training clients and the validation client. In other words a usage pattern that exhibits poor usage cohesion for both the training group and the validation group will be assigned a good consistency value. However at this stage of the validation we want to observe  whether the usage cohesion value are good enough to reveal informative patterns that could be useful for the API documentation. To this end we assessed how many of the eligible pattern (as defined above) retain good value for the usage cohesion regarding the validation client; we considered that these pattern were informative if they retained a PUCv value greater than 0.75. This value was fixed thanks to an observation on a sample of generated pattern. Assessments made at this stage enabled us to answer our second research question \textbf{(RQ2)}.

% \ha{\bf I think we have to remove this paragraph or we have to move it to the Approach section}
%These results and the rest of the experimentation were obtained for the
%following configuration of our algorithm, as explained in Section~\ref{sec:approach} The
%usage pattern are built incrementally, we fixed the relaxing step of the epsilon parameter to 0.05,
%this choice was based on statistical observation of distance between two points for each pair of points in the APIs.
%The second choice we made was to continue the incremental clustering process until epsilon reaches a maximum value witch reflect
%a co-usage similarity of 0.65, this choice was motivated by the will of produce
%clusters that are fairly dense.
% Since we are interested in detecting consistent and cohesive usage patterns, the
% incremental clustering process for identifying usage patterns stops when the epsilon parameter reach a maximal value that we set to 0.35.
% This epsilon threshold means the following: for a given pattern, in the worst cases at least 65\% of the pattern's clients use all the pattern's methods together.

%\ha{I revised the following paragraphs}
%To address our research questions we performed leave-one-out cross-validations.
%In this validation we adopted the following process for all the APIs of the case study.
%\begin{myitemize}
%	\item
%		In the first step, we applied our approach N times on a N-1 client programs for
%		the considered API (N-1 client programs are the training set), leaving away in each time one of the API's client programs as validation set.
%		N being the number of client programs of the considered API in our case-study.
%		The results of this step are N runs, where each run has its associated usage patterns generated with the corresponding training set.
%	\item
%		In the second step, for each run we evaluated the consistency of the generated usage patterns between the training set and the validation set.
%		A pattern is said consistent if the co-usage relationships between the pattern's methods in the context of the training set remain the same (or very similar) in the context of the validation set.
%		It is obvious that in each run only eligible patterns for the validation set are considered for evaluating the consistency.
%		In a given run, a pattern is said eligible if it contains at least one method that is actually used by the run's validation set.
%		However, if only a small subset of the eligible pattern's methods are used by the validation set, while the other methods of this pattern are not used, then the consistency metric that we define in the following --\equref{eq:Consist}-- will evaluate such an eligible pattern as inconsistent.
%\end{myitemize}
%
%To measure the co-usage relationships between the methods of a generated usage pattern we use the Service Usage Cohesion Metric (SIUC), taken from Perepletchikov \etal \cite{Pere07b,Pere10a}.
%%In our definition of consistency we were based on a predefined metric,
%%namely the Service Usage Cohesion Metric (SIUC), taken from Perepletchikov \etal \cite{Pere07b,Pere10a}.
%We use the SIUC since it is a usage cohesion metric and it was recently used in other work \cite{Abde13x,Dani11a} to measure the usage cohesion of interfaces in Java OO applications, where like our definition of a usage pattern, an interface is defined as a group of method declarations.
%However, in this cited body of work the clients of an interface are computed at class granularity (\ie clients are classes), while in our work the clients of a pattern are methods (\ie clients are computed at method granularity).
%In the following, we refer to the SIUC metric as Pattern Usage Cohesion (PUC).
%The metric is defined as:
%
%\begin{equation}
%PUC(p) = \dfrac{\sum_{cm} \dfrac{num\_used\_mtds(p,cm)}{size(p)}}{\vert
%Clients(p)\vert}  \vee cm \in  Clients(p)
%\label{eq:PUC}
%\end{equation}
%Where \textit{cm} denotes a client method of the pattern \textit{p};
%\textit{num\_used\_mtds(p, cm)} is the number of API�s methods which belong to the
%usage pattern \textit{p} and are used by the client method \textit{cm}; and
%$Clients(p)$ is the set of all client methods of the usage pattern \textit{p}.
%$PUC$ takes its value in the range [0..1].
%The larger the value of $PUC$, the better the usage cohesion is.
%$PUC$ states that a usage pattern has an ideal usage cohesion ($PUC = 1$) if all the pattern's methods are actually always used together with regard to all their client methods.
%
%Back to our definition of consistency, the objective is to see whether the detected usage patterns for an  API, based on a set of clients (training set), will behave in a similar way with a new client program of the API (validation client), in terms of their usage cohesion.
%Hence, we define the consistency of a usage pattern as:
%
% \begin{equation}
%Consistency(p) = 1 - \vert PUC_{T}(p) - PUC_{V}(p) \vert
%\label{eq:Consist}
%\end{equation}
%Where  $PUC_{T}$ is the pattern usage cohesion in the context of the training set and $PUC_{V}$ is the pattern usage cohesion in the context of the validation set.
%This metric takes its value in the range [0..1].
%A value close to 1 indicates that the co-usage relationships between the pattern's methods remain the same between training clients and the new validation client, while a value close to 0 indicates a dissimilar behavior between the two sets of clients.
%%It is obvious that these metrics are calculated only for what we call eligible pattern, which is a usage pattern with at least one of its components methods is used in the new client program.
%The results of this step allows us to answer our first research question \textbf{(RQ1)}.
%
%
%
%
%From another perspective, to answer our second research question \textbf{(RQ2)}, we need to evaluate whether detected usage patterns with our technique are enough informative to help in enhancing the API documentation.
%For this purpose, we dissected the consistency metric and we separately observed its two components: the usage cohesion of detected patterns in the context of both training clients (PUCt) and validation clients (PUCv).
%This is necessary because the consistency metric reflects only the behavioral similarity of detected patterns regarding the training clients and the validation client.
%In other words, if a detected usage pattern describes API methods which do not exhibits good co-usage relationships (\ie it is characterized with poor usage cohesion) for both the training clients and the validation clients, this means that this usage pattern is characterized with a good consistency.
%However, such a usage pattern is not informative since it does not provide valuable information regarding co-usage relationships between the API methods.
%Hence, at this stage of the validation, we want to observe whether the usage cohesion of generated usage patterns is good enough to reveal informative patterns that could be useful for the API documentation.
%
%Observing a variety of generated usage patterns for all studied APIs, we found that a usage pattern is informative enough for documenting the co-usage relationships between the API methods if the pattern's usage cohesion value (as measured by \equref{eq:PUC}) is larger than 0.75.
%Indeed, roughly speaking, a $PUC(p)$ value that is equals to 0.75 is interpreted as follows: in average at least $75\%$ of the $p$'s methods are co-used together with regard to all usage contexts of the $p$'s methods.
%Using this threshold for $PUC$'s values, we evaluated the precision of our technique for identifying informative usage patterns by the normalized ratio of generated (eligible) usage patterns which are informative in the context of both training clients (\ie $PUCt > 0.75$) and validation clients (\ie $PUCv > 0.75$).
%
%\ha{I stopped here}
%
%%In the last step of our evaluation we tried to find out to which extent the detected usage patterns was good and informative. For this we dissected the consistency metric and we separately observed its two components PUCt and PUCv.
%%
%%In fact, this was necessary because the consistency metric reflected only the behavioral similarity of the pattern regarding the training clients and the validation client. In other words a usage pattern that exhibits poor usage cohesion for both the training group and the validation group will be assigned a good consistency value. However at this stage of the validation we want to observe  whether the usage cohesion value are good enough to reveal informative patterns that could be useful for the API documentation. To this end we assessed how many of the eligible pattern (as defined above) retain good value for the usage cohesion regarding the validation client; we considered that these pattern were informative if they retained a PUCv value greater than 0.75. This value was fixed thanks to an observation on a sample of generated pattern. Assessments made at this stage enabled us to answer our second research question \textbf{(RQ2)}.
%
%\ha{I've to revise this paragraph also}
%These results and the rest of the experimentation were obtained for the
%following configuration of our algorithm, as explained in Section~\ref{sec:approach} The
%usage pattern are built incrementally, we fixed the relaxing step of the epsilon parameter to 0.05,
%this choice was based on statistical observation of distance between two points for each pair of points in the APIs.
%The second choice we made was to continue the incremental clustering process until epsilon reaches a maximum value witch reflect
%a co-usage similarity of 0.65, this choice was motivated by the will of produce
%clusters that are fairly dense.



==> sections/visualisationTool.tex <==
\subsection{Pattern Visual Exploration} 
With the exponentially growing number of software libraries in the Internet, the size of possible usage patterns tends to be very large. To simplify the exploration of the inferred patterns, we opted for an interactive and user-friendly visual exploration technique. The distribution of libraries
on different usage cohesion levels follows a hierarchical structure by inclusion
that can be visualized through a treemap layout \cite{ johnson1991tree}.
However, to better reveal the hierarchy, we opted for a circle packing visualization \cite{wang2006visualization} even if circle packing is not as space-efficient as a treemap.


In our visualization, the libraries are represented as white dots and the clusters as circular region with deferent shades of blue.  \Figref{fig:visualization} shows an example of the circle packing visualization.
Elements belonging to the same cluster (co-used elements) are placed at the inner periphery of the circular region representing the cluster. Thus the nesting between circular regions indicates the different clustering level.  Our visualization enables us to map different information to the graphical component of the visualization scene. For instance, library popularity can be mapped to the dot size, and the cluster cohesion can be mapped to the region color.


The developer can use our visualization to explore the inferred patterns. The exploration is based only on pattern cohesion and the circle packing nesting.
Our visualization environment provides also an interactive navigation where the user can click on any usage pattern, i.e., cluster, to zoom in or zoom out. The visualization allows also to place the mouse over a library to get a tooltip with
some more information. For example, when clicking on a library the user is redirected automatically to its artefact  home page on the Maven Central repository\footnote{http://mvnrepository.com} in order to download the library jar file.
Our visualization allows also the developer to provide as input the set of libraries he is already using in his system and for which he is trying to find related and commonly used libraries. Thereafter, the entered libraries are highlighted
in a different color, and the developer can start his exploration from the highlighted points.

\begin{figure}[!t]
\centering

	\includegraphics[width=0.95\linewidth]{img/packing.pdf}


\caption{circle packing visualization}
\vspace{-0.25cm}
\label{fig:visualization}
\end{figure}

